Training Deep Neural Networks with Joint Quantization and Pruning of Weights and Activations

Quantization and pruning are core techniques used to reduce the inference costs of deep neural networks. State-of-the-art quantization techniques are currently applied to both the weights and activations; however, pruning is most often applied to only the weights of the network. In this work, we jointly apply novel uniform quantization and unstructured pruning methods to both the weights and activations of deep neural networks during training. Using our methods, we empirically evaluate the currently accepted prune-then-quantize paradigm across a wide range of computer vision tasks and observe a non-commutative nature when applied to both the weights and activations of deep neural networks. Informed by these observations, we articulate the non-commutativity hypothesis: for a given deep neural network being trained for a specific task, there exists an exact training schedule in which quantization and pruning can be introduced to optimize network performance. We identify that this optimal ordering not only exists, but also varies across discriminative and generative tasks. Using the optimal training schedule within our training framework, we demonstrate increased performance per memory footprint over existing solutions.

==> backup/note.tex <==
\section{Introduction}
	
Deep neural networks have been widely deployed in various applications. To
improve the neural network inference efficiency, quantization and pruning
have become the indispensible procedures before the deployment of a network
model. The former reduces the bit-width of weight and feature, which
provides smaller memory footprint and fixed-point arithmetic acceleration.
The latter pruning weight or neurons to produce a sparse network which
requires less memory and computation budget. As we can see in
Sec.~\ref{sec:relate} and appendix~\ref{apn:related_work}, there have been a
great deal of research work in these two directions.
	
Despite many successes, we believe that the current study still have remaining
problems to solve.  
	
\begin{itemize}
	\item[\bsquare] Pruning and quantization are often considered to be able to solve
	      independently \citep{n21_liang2021pruning, o_paupamah2020quantisation},
	      though there have been some recent research to study both quantization and
	      pruning in a unified scope.
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item[\bsquare] Not enough attention has been paid to unstructured
	      pruning on the feature map. Although there are many studies on
	      unstructured and structured weight pruning, we
	      argue that it is far more beneficial for inference if we apply
	      unstructured pruning on feature rather than weight. Take
	      convolution as an example, we can save an entire dot
	      product by only skipping a single output feature value \citep{convarith_dumoulin2016guide}.
	      	      	      	      	      			  
	      %   \citep{h_gemm}
	      %   \citep{h_colbert2021energy,h_jha120data}
	      % \citep{detect_li2019fully}
	      %   \citep{detect_tzelepis2019deep} \citep{detect_wei2018quantization}																																																																																																																																																																																																								  
	\item[\bsquare] Most existing work are focused on classification tasks, and some work have covered
	      object detection \citep{detect_li2019fully}.
	      However, there is still very little pruning and quantization
	      research on generative tasks like generative adversarial networks
	      (GAN) or image to image translation.
	      	      	      	      	      
	      	      	      	      	      																																																																																																																																																																																																																																   
	\item[\bsquare] None of available network compression tools can provide both a
	      set of flexible APIs and joint quantization \& pruning training capability,
	      despite the large number of publications on related directions.
	      	      	      	      	      																																																																																																																																																																																																																																   
\end{itemize}
	
	
Therefore, to solve the above problems, we make the following contributions in
this paper. 
	
\begin{enumerate}
	\item We propose a joint quantization and pruning method, and points out
	      that these two operations are non-commutative and even dependant,
	      instead of independent in certain cases.
	      	      	      	      	      																																																																																																																																																																																																																																  
	      	      	      	      	      	
	\item To the best of our knowledge, this is the first work that studies
	      unstructured feature pruning extensively. We discover it works in a
	      completely different pattern to existing pruning paradigm, which identifies
	      it to be a new and important scenario for model compression
	      research. 
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item We verify our method to have strong performance and robustness on
	      image classification, object detection, super resolution, Pix2Pix
	      \cite{pix2pix} and CycleGAN \citep{o_cyclegan}, where we also
	      discover and summarize many meaningful findings, especially from
	      generative tasks.
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item We release our method as a pytorch-based python package.
	      Contrary to existing libraries like \citep{t_xilinx}, which only
	      provides a limited set of 
	      quantized or pruned modules isolated from other toolchain, 
	      we come up with an entirely innovative design.
	      Our library only exposes two layer-level primitives and works
	      seamlessly with any other pytorch modules.
	      											  
	      											 
	      %   which is
	      %   surprisingly simple by only exposing two layer-level primitives for
	      %   quantization and pruning, and could be easily extended and integrated
	      %   with other use cases.
\end{enumerate}
					
					
					
					
\section{Related Works} 
\label{sec:relate}
				
Due to space limit and the fact that both quantization and pruning are large areas of research
with broad practical impacts, we will only outline concepts and work closely related to our contributions
in this section. We provide a much broader and detailed review in appendix~\ref{apn:related_work}.
				
				
					
\textbf{Quantization.} Quantization \citep{n16_wu2020integer} is the process
of quantifying floating numbers with integer equivalents and can be applied
on both weights and feature. Post-training quantization
\citep{n26_lee2018quantization} aims on converting a trained float network
to quantized version without adequate access to training data, which is
convenient but sometimes suffers from accuracy degradation.
Quantization-aware training \citep{o_hubara2017quantized} involves
quantization into the training process, which usually provides better
accuracy but requires more efforts. Most work are focused on classification
tasks, while there are some recent work \citep{detect_wei2018quantization,
detect_li2019fully} on quantization for objection detection networks.
\citep{n23_wang2019qgan} quantizes the weight of a GAN to low bit-width on
CIFAR10 and CelebA \citep{o_celebA}.
					
				
					
					
\textbf{Pruning.} Sparsity is a long-standing research problem in the neural
network domain \citep{n38_gale2019state, n35_hoefler2021sparsity}, and
pruning is an important technique to obtain sparse neural network by
removing unimportant connections. Finetuning-based methods prune gradually
during training \citep{n45_zhu2017prune}, and retraining-based methods
retrain networks with pruned structure \citep{n37_frankle2018lottery}. There
have been debates about which one is better \citep{n29_liu2018rethinking,
renda2020comparing}. Most of known pruning methods act on weight, and can be
categorized as structured \citep{o_liu2017learning} and unstructured pruning
\citep{o_han2015learning}, while the former one requires to removes a
channel of weight together and the latter one can remove weight arbitrarily.
Most work are focused on classification tasks, and
\citep{detect_he2017channel} proposes a layer-wise structured pruning method
for object detection. There are some work connects GAN with sparsity
\citep{n34_zhou2020sparse}, but their major focus is on how to use sparse
regularization to improve generative quality instead of pruning.
				
				
					
\textbf{Joint Quantization and Pruning.} There are relatively few work that jointly
consider pruning and quantization. Most work assumes a Prune-then-Quantize
pipeline \citep{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint}. 
\citep{n21_liang2021pruning,
n24_paupamah2020quantisation} further claim that pruning and quantization can
be studied independently. 
					
				
					
					
\textbf{Neural Network Compression Toolbox.} There are many open-source
model compression tools that provide pruning or quantization functionality.
However, as far as our best knowledge, none of them offer joint pruning \&
quantization. Moreover, many tools are designed to be heavily inflexible and
some even requires developers to write code in a domain-specific language
(DSL). We discuss this more details in appendix~\ref{apn:related_work}.
					
					
				
					
					
					
\section{Method}
\label{sec:method}
			
Our method has three modules. We explain our pruning and quantization
operators design in Sec.~\ref{sec:quantize_operator} and
\ref{sec:prune_operator}, and a joint pipeline
to collaborate them in structural and temporal dimensions in Sec.~\ref{sec:joint_pip}. We also explain
why not to adopt a commonly used Prune-then-Quantize pattern and how
unstructured feature pruning works.
					
% Our approach consists of three modules. The first two are pruning and
% quantization operators. We design them to be able to work
% independently on both feature and weight. Then we propose a joint pipeline that
% allows two operators to collaborate smoothly.
					
\subsection{Quantization Operator}
\label{sec:quantize_operator}	
			
% algorithm block
% supports channelwise, when apply either on feature/weight can channelwise
					
Our quantization operator is an improved version from
\citep{o_hubara2017quantized}, by which they both leverage "straight-through
estimator" for gradient calculation and follow a inference-friendly linear
quantization scheme \citep{n25_jacob2018quantization}. Giving input $x_t$ to
denote either weight or feature at step $t$, $N$ be the total number of
bits, $d$ be the number of decimal bits\footnote{Bits used to represent
	fractions}, the quantized $x_t$ can be represented by $\hat{x}_t$:
					
					
\begin{equation}
	\begin{split}
		\hat{x}_t & = \text{clip}(\floor{x_t * 2^{d}}, -2^N, 2^N-1) / 2^d \\
		\frac{\partial Loss}{\partial x_t} & = \text{clip}(\frac{\partial Loss}{\partial \hat{x}_t}, -2^{N-d}, 2^{N-d} - 1)
	\end{split}
	\label{eq:quantize}
\end{equation}
					
					
However, we make two simple yet effective enhancements on top of existing methods, as
explained below and Alg.~\ref{alg:quantize}. 
			
% Note we also adopt the per-channel
% quantization scheme from \citep{n28_krishnamoorthi2018quantizing}, thus the
% Alg.~\ref{alg:quantize} can work channelwisely.
					
\begin{enumerate}
	\item \textbf{Delayed Quantization Error Minimization.} Instead of using floating point auxiliary weights for simulated
	      quantization \citep{n25_jacob2018quantization} or finding clever weight
	      initialization \citep{o_init_q}, we start by training the original float network, then calculate the optimal decimal
	      bits by minimizing the quantization error after a given number of
	      steps $t_q$. By thorough experiments in Sec.~\ref{sec:exp}, we
	      shall that it makes our method robust enough
	      to accommodate initialization and training dynamics of various applications.
	      		      		      		      		      																																																																																																																																																																																																																															  
	\item \textbf{Saturated Quantization.} When calculating the optimal decimal bits, instead of using the
	      standard mean square quantization error $\arg \min_{d} |\hat{x}_t - x_t|^2$,
	      we saturate $x_t$ to protect the quantization from outliers:
	      		      		      		      		      																																																																																																																																																																																																																															  
	      \begin{equation}
	      	\begin{split}
	      		d^* & = \arg \min_{d} |\hat{x}_t - \text{saturate}(x_t)|^2 \\
	      		\text{saturate}(x) & = \text{clip}(x, \text{quantile}(x, s_l), \text{quantile}(x, s_u)) \\
	      		\text{quantile}(x, a) & =  a\text{-th quantile of } x \\
	      		s_l, s_u & \in [0, 1], s_l < s_u
	      	\end{split}
	      	\label{eq:qmse}
	      \end{equation}
	      		      		      		      		      																																																																																																																																																																																																																															  
	      Later we show that it is critical for
	      applications like CycleGAN in Fig.~\ref{fig:cyclegan_demo} and Fig.~\ref{fig:feat_histogram}.  % fig:cyclegan_demo
	      		      		      		      		      																																																																																																																																																																																																																															  
	      % \item Similar to the Prune Operator in Alg.~\ref{alg:prune}, we also propose to
	      %       use a buffer to collect a short-term history of $x_t$ instead of only
	      %       relying $x_t$ for the optimization in Eq.~\ref{eq:qmse}.
\end{enumerate}
					
			
				
\subsection{Pruning Operator}
\label{sec:prune_operator}
					
					
Our pruning operator is an improved version from \citep{n45_zhu2017prune}.
Specifically, it is an automated gradual pruning algorithm where the
sparsity is increased during training for $n$ repetitions till the final
sparsity $s_f$. Let $\Delta t$ be the interval between each pruning step,
$t_0$ be the start step of the pruning procedure, the sparsity at time $t$
is denoted by $s_t$ in Eq.~\ref{eq:sparsity}.
					
\begin{equation}
	s_{t}=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta t}\Bigr\rfloor\right)^{3} \right) 
	\label{eq:sparsity}
\end{equation}
					
At each pruning step when $t = t_0 + i \Delta t, i\in [n]$, a mask $m_t$ is
calculated by zeroing out the smallest magnitude input until the $s_t$ is
reached. This mask will be kept the same for both training and inference until
the next pruning step if exists. 
					
The modification we make is instead of only depending on magnitude of the
current input, we maintain an input buffer so we construct the mask from the
magnitude of a history of inputs. Later we see that the input buffer is important for
unstructured feature pruning in Table~\ref{tb:frcnn_main}. 
					
						
\begin{multicols}{2}
	\begin{minipage}{0.49\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\SetNlSkip{0em}
			\KwInput{number of bits $N$, quantize step $t_q$ \\ \hspace{2em} saturation range $s_l,
			s_u$}     % , buffer size $b_s$
			\KwOutput{decimal bits $d$}
			% $B \gets $ empty queue with size $b_s$\\
			$d \gets 0$ \\
			\For{$t \gets 1$ to $T$}{
				\eIf{$t < t_q$}{
					$o_t \gets x_t$	
					}{
					\If{$t\equiv t_q$}{$d \gets $ calculate from $x_t, s_l, s_u$ with Eq.~\ref{eq:qmse}}
					$o_t \gets \text{clip}(\floor{x_t * 2^{d}},$ \\
					\hspace{4em} $-2^N, 2^N-1) / 2^d$
				}
			}
			\caption{Quantize Operator}
			\label{alg:quantize}
		\end{algorithm} 
	\end{minipage}
									
	\begin{minipage}{0.49\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\KwInput{sparsity $s_f$, start step $t_0$, interval $\Delta t$ \\
				\hspace{3em} repetition $n$, buffer size $b_s$}     
			\KwOutput{mask $m_T$}
																																																																																																													
			$B \gets $ empty queue with size $b_s$\\
			$s_0 \gets 0$ and $m_0 \gets \mathbb{1}$ \\
			\For{$t \gets 1$ to $T$}{
				append $x_t$ to B \\
				$s_{t}=s_{f} \Big(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta
					t}\Bigr\rfloor\right)^{3} \Big)$ \\
				\eIf{$s_{t-1} \neq s_t$}{
					$m_t \gets $ calculate mask from $B$ and $s_t$
					}{
					$m_t \gets m_{t-1}$
				} 
				$o_t \gets x_t * m_t$
			}
			\caption{Pruning Operator}
			\label{alg:prune}
		\end{algorithm} 
	\end{minipage}
									
\end{multicols}
					
				
					 
Giving input $x_t$ to denote either weight or feature at step $t$, $T$ as
the total number of steps, $o_t$ to denote the operator output, the pruning
operator mechanism is demonstrated in Alg.~\ref{alg:prune}. The mask
calculation in line 8 will find the positions with smallest magnitude
averaged over a buffer of history inputs.
					
				
					
					
\subsection{Joint Pipeline}
\label{sec:joint_pip}
					
Both prune and quantize operator can work independently on either weight or
feature, it's natural to design a
jointly pruned and quantized layer as shown in Fig.~\ref{fig:pipeline},
where pruning is applied before quantization structurally as
\citep{n17_yu2020joint} has explained the benefit that pruning can help to
reduce quantization error because 0 can always be perfectly quantized. 
However, we point out two previously under-studied perspectives, temporal
collaboration between two operators and unstructured feature pruning.
			
\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\linewidth]{plots/conv.pdf}
	\caption{An example of applying joint pruning and quantization on a
		convolution layer. We use dotted lines for prune operator since it
	is applied either on feature or weight.}
	\label{fig:pipeline}
\end{figure}
			

\subsubsection{Unstructured Feature Pruning}
		
Due to the flexibility of our method, we find it is possible to apply the
prune operator in Alg.~\ref{alg:prune} directly on feature map, which we
call \textit{unstructured feature pruning}. Similar to weight pruning, it
will generate a fixed binary mask for each feature, and masked feature
values will always be zero. To put in an intuitive way of speaking, it is
like having \q{holes} on designated locations of a feature map.

In many ways, unstructured feature pruning is a worthy problem. On the one
hand, unstructured feature pruning is more flexible than structured pruning
\footnote{Structured pruning is equivalent to weight and feature because it
operates per channel.} because it does not have to prune at a per-channel
granularity. On the other hand, unstructured feature pruning can be much
more rewarding for inference than unstructured weight pruning because
skipping a single output value could save an entire dot product.


			
			
\subsubsection{Temporal Collaboration}
					
Temporally, we could jointly schedule two operators by controlling the
relationship between $t_0 + n\Delta t$ in Alg.~\ref{alg:prune} and $t_q$ in
Alg.~\ref{alg:quantize}. Previous methods generally assume a
Prune-then-Quantize paradigm ($t_0 + n\Delta t > t_q$) without much
scrutiny. However, we find this argument is not sufficient to encompass the
relationship between pruning and quantization when taking unstructured
feature pruning into consideration. 
					
\begin{itemize}
	\item \textbf{Non-Commutativity.} Although many experiments in Sec.~\ref{sec:exp} demonstrate that
	      Prune-then-Quantize temporally provides a better accuracy. 
	      However, in these cases, we find Quantize-then-Prune has a much
	      worse performance on feature pruning scenario. It indicates a
	      non-commutative property between quantization and pruning, which
	      is not discussed by previous methods.
	      		      		      		      		      	
	      		      		      		      		      	
	\item \textbf{Quantize-Then-Prune.} In Sec.~\ref{sec:exp_sr}, we find a reversed relationship where
	      Quantize-then-Prune actually brings much better performance.
	      
	      %   Prune-then-Quantize almost fails to converge. 
	      			 
	      %   Moreover, in addition to non-commutativity, quantization even
	      %   improves feature pruning by a large margin, which is totally
	      %   contrary to our intuition.
	\item \textbf{Quantize-Help-Prune.} In Sec.~\ref{sec:exp_sr}, we even
	      observe that quantization is critical for feature pruning, and feature
	      pruning alone almost fails to converge.
\end{itemize}
					
\textbf{Gradient Peak Effect.} Furthermore, we provide a gradient
perspective to explain these phenomena. As shown in
Fig.~\ref{fig:why_prune_then_quantize}, we find that pruning will incur
spikes on gradient of activations when operating on feature because loss
will be more concentrated on the remaining values. We suppose this could
even be exacerbated through back-propagation. Moreover, the gradient peak
could correlate with two additional dynamics: (1) the gradient clamping from
straight-through gradient estimator in Eq.~\ref{eq:quantize}. (2) gradient
of the origin model. We could obtain various training results when
the tension among these dynamics goes differently. 
	
Therefore, we show that unstructured feature pruning works in a
completely different pattern to existing pruning paradigms, which we believe
could identify it to be a practical scenario for model compression research.
Based on our findings, we propose pruning and quantization to collaborate
temporally but not in a pre-defined manner.
	


\section{Software Interface}
					

We release our method in a pytorch-based software package. In
Listing~\ref{code:interface}, we demonstrate how simple and flexible it can
make for pruned and quantized training. Unlike existing libraries
\citep{t_xilinx,QatTorch}, we propose a novel design which directly
transforms the weight attribute of the input layer into a pruned or
quantized version during runtime. This is to say, our library is
layer-agnostic and can work with any pytorch modules, as long as their
parameters can be accessed from the weight attribute. Additionally, it
leaves the original weight and bias untouched. Users won't even need to
change weight initialization code for pruned and quantized training.
More information can be found at \ourlib.


					
\begin{listing}[]
	\python{snippets/interface.py}
	\vspace{-2.5em}
	\caption{Examples to demonstrate our software interface for quantization and pruning}
	\label{code:interface}
\end{listing}
					
					
					
\section{Experiments}
					
\label{sec:exp}
					
To evaluate our method, we conduct experiments on five tasks: image
classification, object detection, super resolution, image to image translation,
and generative adversarial network. 
	
For each task, if not specifically stated, we apply 8-bit quantization on
both feature and weight of every layer, unstructured pruning with sparsity
of 50\% on either feature or weight except for the first \& last layer.
For a simpler notation, we use abbreviation to represent each experiment
configuration as summarized in Table.~\ref{tb:abbr}.
					
					
\begin{table}[H]
	% \scriptsize
	\centering
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Abbreviation} & \textbf{Description}                                                   \\ \hline
		Q                     & Quantize all features and weights with 8 bits                          
		\\ \hline
		P (W/F)               & P (W) means to prune 50\% weights, and P(F) means prune 50\% features. \\ \hline
		P-Q / Q-P             & P-Q means to apply pruning and then quantization                       
		temporally, Q-P means   the opposite.         \\ \hline
		BF                    & Buffer size in Alg.~\ref{alg:prune}, BF=1 means $b_s=1$.               \\ \hline
		W/F Bits              & Bits for weight or feature                                             \\ \hline
		W/F Sparsity          & Ratio of fixed zeros in weight or feature map                          \\ \hline
		Reference/Ref         & Dense and floating point model.                                        \\ \hline
		--                    & Not applicable, e.g., F Sparsity will be `--' for methods don't        
		apply feature pruning. \\ \hline
	\end{tabular}
										
	\caption{Description for experiment configuration abbreviations}
	\label{tb:abbr}
\end{table}
					
We implement each task by applying minimal code changes with our library
on top of existing popular open-source implementations. 
We maintain most hyper-parameters identical to the original settings except for 
training epochs and when to apply quantization \& pruning. 
We provide more details about experiment setups in
appendix~\ref{apn:detailed_exp}. We release all experiment source code as
examples for our library.
					
					
					
\subsection{Image Classification}
					
					
We conduct our image classification task on CIFAR10 \citep{o_cifar10} with
MobileNetV2 \citep{mobilenetv2}, Results of different configurations are shown
in Table~\ref{tb:cls_main}. We compare with previous methods in
Table~\ref{tb:cifar10_comp}. We basically have no accuracy loss in Q and P(W).
Even in the case of both feature pruning and quantization, we only suffer a
minor loss of less than 1.
					

\begin{table}[]
	\centering
	% \vspace{-0.5em}
	\begin{tabular}{rrrrrrrrrrr}
		\hline
		& Ref & Q  & P  (W) & P  (F) & P-Q (F) & P-Q (W) & Q-P
		(F) & Q-P (W)   \\
		\hline
		Accuracy & 92.6 & 92.52 & 92.58 & 91.87 & 91.65 & 92.23 & 88.17 & 85.94  \\
		\hline
	\end{tabular}
	\caption{Validation accuracy with different prune \& quantization
	configurations on CIFAR10. Q-P performs
	much worse than P-Q, which indicates a non-commutative
	property between quantization and pruning. }
	\label{tb:cls_main}
	\vspace{-1.5em}
\end{table}
	
				
					
\begin{table}[]
	\centering
	\vspace{-1em}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccccccl}
			\toprule
			Method                                                                        & Network                                           & W Bits                    & F Bits                   & W Sparsity                  & F Sparsity                & Ref Accuracy                               & \multicolumn{1}{c}{Accuracy}      \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n2_yang2020automatic}}}                    & \multicolumn{1}{c|}{ResNet-20}                    & \multicolumn{1}{c|}{1.9}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{91.29}                 & 91.15 (-0.14)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n3_xiao2019autoprune}}}                    & \multicolumn{1}{c|}{VGG-16}                       & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{79\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.4}                  & 91.5 (-1.9)                       \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n4_van2020bayesian}} }                     & \multicolumn{1}{c|}{VGG-7}                        & \multicolumn{1}{c|}{4.75} & \multicolumn{1}{c|}{5.4} & \multicolumn{1}{c|}{0\%}    & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.05}                 & 93.23 (+0.18)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n24_paupamah2020quantisation}}}            & \multicolumn{1}{c|}{MobileNet}                    & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{37.5\%} & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{91.31}                 & 90.59 (-0.72)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{3}{*}{\script{\citep{n29_liu2018rethinking}}}}  & \multicolumn{1}{c|}{VGG-19}                       & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{80\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.5}                  & 93.52 (+0.02)                     \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{PreResNet-110}                & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.04}                 & 95.06 (+0.02)                     \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{DenseNet-100}                 & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.24}                 & 95.21 (-0.03)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{2}{*}{\script{\citep{n33_dettmers2019sparse}}}} & \multicolumn{1}{c|}{VGG16-C}                      & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.51}                 & 93 (-0.51)                        \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{WRN-22-8}                     & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.74}                 & 95.07 (-0.67)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n40_choi2016towards}}}                     & \multicolumn{1}{c|}{ResNet-32}                    & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{77.8\%} & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.58}                 & 92.64 (+0.06)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n41_choi2020universal}}}                   & \multicolumn{1}{c|}{ResNet-32}                    & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{7.3\%}  & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.58}                 & 92.06 (-0.52)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n43_zhao2019variational}}}                   & \multicolumn{1}{c|}{ResNet-20}                        & \multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{16.47\%} & \multicolumn{1}{c|}{16.47\%\footnote{It has a sparse feature
			because it applies structured pruning on weight, which corresponds to
			channel pruning on feature.}} & \multicolumn{1}{c|}{92.01}                 & 91.66 (-0.35)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n44_achterhold2018variational}}}           & \multicolumn{1}{c|}{DenseNet-76}                  & \multicolumn{1}{c|}{2}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.19}                 & 91.17 (-1.02)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{5}{*}{Ours}}                                    & \multicolumn{1}{c|}{\multirow{5}{*}{MobileNetV2}} & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{\multirow{5}{*}{92.6}} & \multicolumn{1}{c}{92.52 (-0.08)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{50\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.58 (-0.02)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{50\%} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.87 (-0.73)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{50\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.23 (-0.37)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{50\%} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.65 (-0.95)} \\ \bottomrule
		\end{tabular}
	} 
	
	\caption[Caption for LOF]{Comparisons with previous pruning or quantization methods on
	CIFAR10. We argue our method stands strongly in performance against existing
	methods, but is far more versatile and robust\footnotemark.}
	\label{tb:cifar10_comp}
	% \vspace{-1em}
\end{table}

			

\footnotetext{Note that it is
	inherently difficult to compare different quantization and pruning methods
	because of diversity and difference between configurations. We continue this
	discussion in appendix~\ref{apn:benchmark}.}
					
					
					
					
					
\subsection{Object Detection}
\label{sec:exp_detection}
					
We conduct our objection detection experiment on Pascal VOC \citep{o_pascalvoc}
using Faster RCNN \citep{o_fasterrcnn} with a ImageNet \citep{o_imagenet}
pre-trained ResNet101 backbone. Since the original Faster RCNN trains on
images of different shapes each batch, it is impossible to obtain a fixed
unstructured pruning mask for convolution feature map as line 8 in
Alg.~\ref{alg:quantize}. Thus, for convolution feature, we apply structured
pruning. Note that we do not prune or quantize for the first 5
residual blocks because they are frozen originally and unfreezing
will collapse the training even for reference network. However, this
limitation can be easily overcome with group normalization or synchronized
batch normalization according to \citep{he2019rethinking}. Thus, we do not
regard this as our limitation.


Results of different configurations are shown in Table~\ref{tb:frcnn_main}. 
We compare with previous methods in Table~\ref{tb:frcnn_comp}. Contrary to existing methods like
\citep{detect_li2019fully}, which introduces major overhauls over the object
detection network training procedures, our method is less intrusive and works
without much modifications. Aligning with the original setting, we train with batch size equal to 1 and fix all
pre-trained batch normalization layers.
					
					
% \textbf{Performance.} It can be seen that we have the smallest performance
% loss among other methods, even when weight \& feature are quantized and weight
% are pruned 50\% (P-Q (W)). In the case of P-Q (F), we suffer a mAP drop of
% 1.47, but this is still smaller than that of
% \citep{n28_krishnamoorthi2018quantizing, detect_he2017channel}.
					 
% \textbf{Robustness.} Contrary to existing methods like
% \citep{detect_li2019fully}, which introduces major overhauls over the object
% detection network training procedures. Our method is less intrusive and works
% without much modifications. Aligning with the original setting, we train with batch size equal to 1 and fix all
% pre-trained batch normalization layers. Note that we do not prune or quantize for the first 5
% residual blocks because they are frozen originally and unfreezing
% will collapse the training even for reference network. However, this
% limitation can be easily discarded as long as group normalization or synchronized
% batch normalization according to \citep{he2019rethinking}. Thus, we do not
% regard this as our limitation.
					
% \textbf{Effect of Buffer Size.} From Table~\ref{tb:frcnn_main}, we can see that
% the mAP will drop 0.4 from P-Q (F) if we set $b_s$ to 1, which indicates that
% decimal bits $d$ and pruning mask $m$ can be more accurately computed from
% multiple batches especially when original batch size is small. 
					
% Furthermore, the training results are well reckoned in the summary 1.(a), 1.(c).
					
					
					  
\begin{table}[]
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{lrrrrrrrrr}
		\hline
		    & Reference & Q     & P  (W) & P  (F) & P-Q (F) & P-Q (F, BF=1) & P-Q (W) & Q-P (F) & Q-P (W) \\
		\hline
		MAP & 74.47     & 74.25 & 74.33  & 73.04  & 73      & 72.6          & 74.44   & 70.13   & 74.13   \\
		\hline
	\end{tabular}
	} \caption{Faster RCNN results with different prune \& quantization
	configurations on Pascal VOC 2007 test set. The
	non-commutativity persists in unstructured feature pruning.}
	\label{tb:frcnn_main}
\end{table}

	  
					  
\begin{table}[]
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{@{}cccccccc@{}}
		\toprule
		Method                           & Detection Framework          & W Bits & F Bits & W Sparsity & F Sparsity & Reference mAP          & mAP           \\ \midrule
		\script{\citep{n26_lee2018quantization}} & YOLO-v2                      & 8      & 8      & --         & --         & 72.64                  & 72.5 (-0.14)  \\ \midrule
		\script{\citep{n27_yang2019quantization}} & SSD
		& 7      & 8      & --         & --         & 77.8                   &
		76.1 (-1.7)   \\ \midrule
		\script{\citep{detect_he2017channel}}  & Faster RCNN & -- & -- & --  & 50\% & 68.7
		& 66.9 (-1.8) \\ \midrule
		\script{\citep{detect_wei2018quantization}}  & Faster RCNN & 8 & 8 & --  & -- &
		44.6	  & 47.0 (+2.4) \\ \midrule
		\script{\citep{detect_yin2016quantization}}  & R-FCN & 6 & -- & --  & -- & 78.94
		& 78.24 (-0.7) \\ \midrule
		\multirow{3}{*}{Ours}            & \multirow{3}{*}{Faster RCNN} & 8      & 8      & --         & --         & \multirow{3}{*}{74.47} & 74.25 (-0.22) \\
		                                 &                              & 8      & 8      & 50\%       & --         &                        & 74.44 (-0.03) \\
		                                 &                              & 8      & 8      & --         & 50\%       &                        & 73 (-1.47)    \\ \bottomrule
	\end{tabular}
	} \caption{Comparisons with previous pruning or quantization methods on
	Pascal VOC 2007. We have the smallest performance loss among other methods.}
	\label{tb:frcnn_comp}
\end{table}

		  
					
\subsection{Super Resolution}
					
\label{sec:exp_sr}
					
We conduct our super resolution task on 91-image \citep{o_91image} (training set)
and Set5 \citep{o_set5} (validation set) with efficient sub-pixel convolution
network (ESPCN) \citep{espcn}, which is a 3-layer convolution network without
normalization layer. Results are summarized in Table~\ref{tb:sr_main}. Though every configuration
suffers a performance drop, our results still have better PSNR than the
original result reported in \citep{espcn} except for unstructured feature pruning cases.

% Note that we find the training is not stable enough.
% Therefore, for each configuration, we run five times and peak the best model, and
% the results are shown in Table~\ref{tb:sr_main}. 
					

					
% \textbf{Quantize helps Feature Pruning.} In this case, not only we find that it
% is more beneficial to quantize first and then prune, we also observe that
% feature pruning yields better performance with quantization. It indicates that
% the non-trivial relationship between quantization and feature pruning as we
% discussed in Sec.~\ref{sec:joint_pip}. This corresponds to summary 1.(c).
					
% \textbf{Gradient Peak.} In Fig.~\ref{fig:why_prune_then_quantize}, we show that
% feature pruning will incur gradient peaks. It is intuitive from hindsight since
% the network is trying to learn more by having large gradients when fractions of
% features suddenly become zero. This corresponds to summary 1.(b). 
					
\begin{table}[]
	\footnotesize
	\centering
	\begin{tabular}{rrrrrrrrrr}
		\hline
		Ref   & Q     & P  (W) & P  (F) & P-Q (W) & P-Q (F) & Q-P (W) & Q-P (F) \\
																	
		\hline
		32.86 & 32.69 & 32.77  & 31.52  & 32.57   & 31.7    & 32.59   & 32.12   \\
		\hline
	\end{tabular}
	\caption{PSNR (peek signal-to-noise ratio) with different prune \&
	quantization configurations on Set5. 
	In this experiment, we find the prune-then-quantize pattern is reversed and
	non-commutativity still holds. Moreover, quantization can even help unstructured feature
	pruning.}
	\label{tb:sr_main}
\end{table}
					
					
					
					
\begin{figure}[]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_feat.pdf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_grad.pdf}
		}
	\end{minipage}
																																						
	\caption{Take the super resolution task as an example, we visualize the
	gradient peak effect during unstructured feature pruning. This phenomenon is
	natural by hindsight and we consider it is generalizable to more scenarios.
	Gradients are sampled from feature.}
	\label{fig:why_prune_then_quantize}
\end{figure}
					
					
					
					
					
					
					
					
\subsection{Image to Image Translation and Generative Adversarial Network}
					
We conduct our image to image translation task on facades dataset with Pix2Pix
network \citep{pix2pix}, and our GAN task on horse2zebra dataset with CycleGAN
\citep{o_cyclegan}. Both of them applies an encoder-decoder structured network,
while the Pix2Pix uses UNet \citep{unet} and CycleGAN uses a variant of ResNet
with deconvolution layers. In Fig.~\ref{fig:pix2pix_demo} and
\ref{fig:cyclegan_demo}, we demonstrate some generated samples, and we provide
more samples in appendix~\ref{apn:more_demos}.
					
From Fig.~\ref{fig:pix2pix_demo}, it is hard to
distinguish the quality difference between the reference and quantized only
network, despite some color difference. If we add weight pruning, we can observe
some details get blurry. However, if we prune feature, though the overall
structure remains, the color becomes unnatural and some major distortions could
be spotted. From Fig.~\ref{fig:cyclegan_demo}, we can find that weight pruned
network transfers the texture correct but the color transfer seems unfinished,
while the feature pruned network looks like the opposite, which may represent a
division of functions within the network. 
					
\textbf{Feature Distribution and Information Granularity.} From
Fig.~\ref{fig:feat_histogram} and \ref{fig:cyclegan_demo} about CycleGAN, we are
amazed to discover that its feature distribution has a much longer tail, and its
generative quality is very sensitive to minor changes in feature, which
corresponds to to summary 2.
					
\begin{figure}[]
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.26}{
			\includegraphics{plots/pictures/pix2pix/main33/24.pdf}
		}
		\caption{Examples of generated images from Pix2Pix networks with different
		configurations. }
		\label{fig:pix2pix_demo}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.26}{
			\inputpgf{plots/pictures/cyclegan/main}{3.pgf}
		}
		\caption{Examples of generated images from CycleGAN networks with different
			configurations. 
			It is clear to see the saturated quantization works as an important factor,
		and more than 8 bits are required for this generative task.}
		\label{fig:cyclegan_demo}
	\end{minipage} 
\end{figure}
					
					
					
					
					
\begin{figure}[]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/feat_histogram_analysis/sr.pdf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/feat_histogram_analysis/cycle.pdf}
		}
	\end{minipage}
	\caption{Feature histogram comparison between the network of super
		resolution and CycleGAN. The features of
		CycleGAN are much more long-tailed, and our saturated quantization can
	handle well. }
	% 	Note that it is also natural to consider logarithmic
	% 	quantization for long-tailed distribution \citep{o_hubara2017quantized},
	% but it may result in additional difficulty for inference acceleration.
	\label{fig:feat_histogram}
\end{figure}
					
					
					
					
\section{Conclusion}
					
In this paper, we design a joint quantization and pruning methods, uncover
unstructured feature pruning as an important scenario for model compression
research and release our method as a software package. Moreover, we conduct
thorough experiments on a wide range of tasks and discover many interesting
findings.
					
Admittedly, this work bears its own limitations. We still could not fully
explain the complex inter-dependency between feature pruning and quantization,
and feature distribution of generative adversarial networks. Feature pruning
still suffers from non-negligible performance drop. However, we believe these
limitations could be regarded as future possibilities. It will be interesting to
see what could be built upon our findings.
					

==> include.backup0922/author.tex <==
\title{Quantized Sparse: Joint Quantization and Pruning Training in Python}


\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@ucsd.edu}
	\And
	Ian Colbert\\
	UC San Diego\\
	\texttt{icolbert@ucsd.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@ucsd.edu} \\
	\And
	Srinjoy Das\\
	UC San Diego\\
	\texttt{s2das@ucsd.edu} 
}

\hypersetup{
pdftitle={Quantized Sparse: Joint Quantization and Pruning Training in Python},
pdfsubject={deep learning},
pdfauthor={Xinyu Zhang},
pdfkeywords={Quantization, Neural Networks, Pruning, Software Tool, Python, Pytorch, Model
Compression, Object Detection, Super Resolution, Classification, Image to Image
Translation, Generative Adversarial Network, CycleGAN},
}

==> include.backup0922/body.tex <==

\begin{abstract}

	In this paper, we propose a joint quantization and pruning method on both
	feature and weight. With our method, we study unstructured feature pruning extensively and
	uncover it to be an important yet overlooked problem for model compression
	research. We verify our method to have strong performance and robustness through
	experiments on image classification, object detection, super resolution, image
	to image translation, and generative adversarial network. Furthermore, we
	release our method as a pytorch-based python package at
	\href{https://todo.com}{https://pypi.org/project/qsparse}, which is surprisingly
	simple and flexible to accommodate various use cases.
	
	\end{abstract}
	
	
	
	\section{Introduction}
	
	Deep neural networks have been widely deployed in various applications. To
	improve the neural network inference efficiency, quantization and pruning have
	become the indispensible procedures before the deployment of a network model.
	The former reduces the bit-width of weights and activations of neural networks,
	which not only reduces the memory footprints but also accelerate computation
	because of the fixed point arithmetic. The latter pruning weights or neurons to
	produce a sparse network which requires less memory and computation budget. As
	we can see in Sec.~\ref{sec:relate}, there have been a great deal of research work in these two
	directions.
	
	Despite many successes, we believe that the current study still have remaining
	problems to solve.  
	
	\begin{itemize}
		\item[\bsquare] Pruning and quantization are often considered to be able to solve
			  independently \cite{n21_liang2021pruning, o_paupamah2020quantisation},
			  though there have been some recent research to study both quantization and
			  pruning in a unified scope
			  \cite{n10_zhao2019focused,n5_tung2018clip,n4_van2020bayesian}.
																																																																																																																																																																																																																															  
		\item[\bsquare] Not enough
			  attention has been paid to unstructured pruning on the feature map, though 
			  there are many studies on unstructured and structured weight pruning
			  \cite{n35_hoefler2021sparsity,n29_liu2018rethinking}.
			  However, it is plausible that unstructured feature pruning is more
			  beneficial for inference than unstructured weight pruning
			  \cite{h_colbert2021energy,h_jha120data} while more flexible than structured
			  pruning \footnote{Structured pruning is equivalent to weight and feature
			  because it operates channelwise.}. Analogous to matrix multiplication, we can save an entire dot
			  product by only skipping a single output feature value \cite{h_gemm}.
																																																																																																																																																																																																																															  
		\item[\bsquare] Most existing work are focused on classification tasks on
			  \cite{o_mnist,o_cifar10,o_imagenet}. Although classification task is a good
			  test bed, it far falls behind to fully meet practical demands. We believe that
			  expanding the research to cover more practical applications, such as object
			  detection \cite{o_fasterrcnn}, generative adversarial networks (GAN)
			  \cite{o_gan,o_cyclegan} and
			  etc, is also academically challenging and needed.
																																																																																																																																																																																																																																   
		\item[\bsquare] None of available network compression tools can provide both a
			  set of flexible APIs and joint quantization \& pruning training capability,
			  despite the large number of them, e.g., \cite{t_intel,t_xilinx}.
																																																																																																																																																																																																																																   
	\end{itemize}
	
	
	Therefore, to solve the above problems, we make the following contributions in
	this paper. 
	
	\begin{enumerate}
		\item We propose a joint quantization and pruning method, and explain why
			  these two operations are non-commutative in certain cases, which
			  indicates that they are not independent for granted.
																																																																																																																																																																																																																																  
	
		\item We study unstructured feature pruning extensively and find it works
		consistently differently than previous pruning paradigms. We believe that we
		identify a new and important scenario for model compression research. 
																																																																																																																																																																																																																															  
		\item We experiment our method on image classification, object detection,
			  super resolution, image to image translation and generative
			  adversarial network (GAN). In addition to verifying our method, we
			  discover and summarize many meaningful findings. 
																																																																																																																																																																																																																															  
		\item We release our method as a pytorch-based python package at
			  \href{https://todo.com}{https://pypi.org/project/qsparse}, which is
			  surprisingly simple by only exposing two layer-level primitives for
			  quantization and pruning, and could be easily extended and integrated
			  with other use cases.
	\end{enumerate}
	
	
	
	
	\section{Related Works} 
	\label{sec:relate}
	
	\textbf{Quantization.} Quantization is the process of quantifying floating
	numbers with integer equivalents. Quantization can be applied on both weights
	and feature, which can then be used for integer arithmetic. Post-training
	quantization operates on a trained network, which is usually more convenient for
	deployment but sometimes suffers from accuracy degradation. Quantization-aware
	training involves quantization into the training process, which provides better
	accuracy but requires to change the original floating point training pipeline.
	\cite{n28_krishnamoorthi2018quantizing, n16_wu2020integer} conduct comprehensive
	quantization experiments for various applications and proposes best practices
	and workflows.
	
	For post-training quantization, \cite{n1_stock2019and} proposes to reduce
	reconstruction loss for in-domain inputs which only needs unlabeled data.
	\cite{n11_xu2020generative, n12_he2021generative} uses GAN to generate fake data
	for post-training quantization. \cite{n15_zhao2019improving} presents a
	channel-splitting method to handle outliers during quantization.
	\cite{n26_lee2018quantization} also leverages channel-level distribution, but it
	conducts experiments on objection detection with  YOLO-v2 \cite{o_yolov2}. For
	quantization-aware training, \cite{o_hubara2017quantized} proposes straight
	through gradient estimator to calculate gradients for quantization layer.
	\cite{n25_jacob2018quantization} inserts simulated quantization operator into an
	existing network during training. \cite{n27_yang2019quantization} studies the
	relation between quantization  and non-linear activation function.
	\cite{n40_choi2016towards} introduces hessian distortion to measure quantization
	error. \cite{n41_choi2020universal} applies the idea of randomized lattice
	quantization to neural network. \cite{n44_achterhold2018variational} formulates
	quantization as a variational inference problem and trains with stochastic
	weight and quantize afterwards. \cite{detect_wei2018quantization} conduct
	quantization and distillation on tiny object detection networks.
	\cite{detect_li2019fully} presents a set of training stabilizing methods for
	quantizing object detection networks. \cite{n23_wang2019qgan} designs an EM algorithm
	to quantize the weight of a GAN to low bit-width on \cite{o_cifar10, o_celebA}.
	
	
	
	\textbf{Pruning.} Sparsity is a long-standing research problem in the neural
	network domain \cite{n38_gale2019state, n35_hoefler2021sparsity}, and pruning is
	one of the most important technique to obtain sparse neural network by removing
	unimportant connections.
	\cite{n3_xiao2019autoprune} proposes to prune by optimizing auxiliary
	parameters. \cite{n6_venkatesan2020out} uses weight rewinds as a retraining
	technique during pruning. \cite{n14_molchanov2019importance} estimates weight
	importance to final loss using taylor expansion to guide pruning selection.
	\cite{detect_he2017channel} proposes a layer-wise constraint-based channel
	pruning method.
	\cite{n22_yeom2021pruning} prunes by relevance score from
	\cite{o_bach2015pixel}. \cite{n37_frankle2018lottery, n30_evci2020rigging}
	claims training network from scratch with pruned structure yields better
	performance. \cite{n39_luo2017thinet} presents a method to prune layer-wisely
	based on statistics of next layer. \cite{n43_zhao2019variational} designs a
	variational inference method to estimate channel importance for pruning.
	\cite{n45_zhu2017prune} proposes a stage-wise pruning method with an annealing
	process. \cite{n46_chen2018constraint} also designs an annealing pruning
	procedure under constrained bayesian optimization perspective.
	
	
	All of the above methods are for weight pruning, and can be categorized as
	structured \cite{o_liu2017learning} and unstructured pruning \cite{o_han2015learning}, while the former one requires to remove a
	group of weights together, i.e. channel-wise pruning.
	\cite{n29_liu2018rethinking} finds that structured pruning is equivalent to an implicit
	neural architecture search but its margin over random pruning is limited. There
	are some work connects GAN with sparsity
	\cite{n32_mahdizadehaghdam2019sparse, n33_dettmers2019sparse,
	n34_zhou2020sparse}, but their major focus is on how to use sparse
	regularization to improve generative quality.
	
	
	\textbf{Joint Quantization and Pruning.} There are not many work that jointly
	consider pruning and quantization. \cite{n21_liang2021pruning,
	n24_paupamah2020quantisation} claim that they can be studied independently.
	\cite{n5_tung2018clip}
	focuses on training acceleration for pruning and quantization instead of
	accuracy.
	\cite{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint} study methods that
	prune and quantize weight while ignoring feature. \cite{n17_yu2020joint} also
	advices pruning shall happens before quantization but merely from the
	quantization error perspective.
	\cite{n4_van2020bayesian} presents an integer optimization inspired
	method that quantizes weight \& feature, and prunes weight, but it does not
	study feature pruning nor does it discloses its implementation.
	\cite{detect_tzelepis2019deep} proposes a dynamical clustering based model
	compression method with pruning and quantization and conduct experiments on
	object detection tasks, but does not report detailed resulting accuracy.
	
	
	
	\textbf{Neural Network Compression Toolbox.} There are many open-source or
	proprietary neural network compression tools that provide pruning or
	quantization functionality. However, as far as our best knowledge, none of them
	offer joint pruning \& quantization on both weight and feature. Moreover, many
	tools are designed to be heavy and requires developers to write code in a
	domain-specific language (DSL), which is highly inflexible.
	
	
	\cite{t_intel} is one of the most comprehensive tool, which supports both
	pruning and quantization, but it does not provide joint-training examples. It
	also requires writing complex schedule files in order to train models.
	\cite{AiMet} implements a set of pruning and quantization methods separately and
	provides few examples. \cite{TorchPruning} only has structured pruning.
	\cite{n10_zhao2019focused} provides a joint method implementation, but it only
	works on weight and it ships with a set of obscure DSL.
	\cite{n18_shah2020kd} includes module-level API on pruning and quantization
	individually. \cite{t_xilinx} has a set of layer-level neural network API, which
	is more flexible, but it only provides quantization-aware training, and later we
	will see our API design is much simpler and versatile. PyTorch
	\cite{t_paszke2019pytorch} has built-in support for both functions, but
	\cite{QuantizationTorch,PruneTorch} only works on module-level and has limited
	support on quantization-aware training \cite{QatTorch}. \cite{TensorRT}
	provides post-training quantization only and mainly focuses on its efficient CUDA
	inference library. 
	
	
	
	
	\section{Method}
	\label{sec:method}
	
	Our approach consists of three modules. The first two are pruning and
	quantization operators. We design them to be able to work
	independently on both feature and weight. Then we propose a joint pipeline that
	allows two operators to collaborate smoothly.
	
	
	\subsection{Pruning Operator}
	\label{sec:prune_operator}
	
	
	Our pruning operator is an improved version from \cite{n45_zhu2017prune} with a
	simple modification. Specifically, it is an automated gradual pruning algorithm
	where the sparsity is increased during training for $n$ repetitions till the
	final sparsity $s_f$. Let $\Delta t$ be the interval between each pruning step,
	$t_0$ be the start step of the pruning procedure, the sparsity at time $t$ is
	denoted by $s_t$ in Eq.~\ref{eq:sparsity}.
	
	\begin{equation}
		s_{t}=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta t}\Bigr\rfloor\right)^{3} \right) 
		\label{eq:sparsity}
	\end{equation}
	
	At each pruning step when $t = t_0 + i \Delta t, i\in [n]$, a mask $m_t$ is
	calculated by zeroing out the smallest magnitude input until the $s_t$ is
	reached. This mask will be kept the same for both training and inference until
	the next pruning step if exists. 
	
	The modification we make is instead of only depending on magnitude of the
	current input, we maintain an input buffer so we construct the mask from the
	magnitude of a history of inputs. Though it may seem like a small improvement,
	later we see that this is critical for unstructured feature pruning in
	Table~\ref{tb:frcnn_main}. 
	
	
	\begin{algorithm}[H]
		\SetAlgoLined
		\KwInput{sparsity $s_f$, start step $t_0$, interval $\Delta t$,
		repetition $n$, buffer size $b_s$}     
		\KwOutput{mask $m_T$}
																																																																																										
		$B \gets $ empty queue with size $b_s$\\
		$s_0 \gets 0$ \\
		$m_0 \gets \mathbb{1}$ \\
		\For{$t \gets 1$ to $T$}{
			append $x_t$ to B \\
			$s_{t}=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta
				t}\Bigr\rfloor\right)^{3} \right)$ \\
			\eIf{$s_{t-1} \neq s_t$}{
				$m_t \gets $ mask calculation from $B$ and $s_t$
				}{
				$m_t \gets m_{t-1}$
			} 
			$o_t \gets x_t * m_t$
		}
		\caption{Pruning Operator}
		\label{alg:prune}
	\end{algorithm} 
	 
	Giving input $x_t$ to denote either weight or feature at step $t$, $T$ as the
	total number of steps, $o_t$ to denote the operator output, the pruning operator
	mechanism is demonstrated in Alg.~\ref{alg:prune}. The mask calculation in line
	8 will find the positions with smallest magnitude averaged over a buffer of
	inputs, which can be extended to support both unstructured and structured
	pruning, as shown in Sec.~\ref{sec:exp_detection}.
	
	
	
	
	\subsection{Quantization Operator}
	
	% algorithm block
	% supports channelwise, when apply either on feature/weight can channelwise
	
	Our quantization operator is an improved version from
	\cite{o_hubara2017quantized}, by which they both leverage "straight-through
	estimator" for gradient calculation and follow a linear quantization scheme like
	in \cite{n25_jacob2018quantization},
	which is integer arithmetic friendly. Giving input $x_t$ to denote either weight
	or feature at step $t$, $N$ be the total number of bits, $d$ be the number of
	decimal bits\footnote{Bits used to represent fractions}
	, the quantized $x_t$ can be represented by $\hat{x}_t$:
	
	
	\begin{equation}
		\begin{split}
			\hat{x}_t & = \text{clip}(\floor{x_t * 2^{d}}, -2^N, 2^N-1) / 2^d \\
			\frac{\partial L}{\partial x_t} & = \text{clip}(\frac{\partial L}{\partial \hat{x}_t}, -2^{N-d}, 2^{N-d} - 1)
		\end{split}
		\label{eq:quantize}
	\end{equation}
	
	
	We make several enhancements on top of existing methods, which are explained in
	the following and Alg.~\ref{alg:quantize}. Note we also adopt the per-channel
	quantization scheme from \cite{n28_krishnamoorthi2018quantizing}, thus the
	Alg.~\ref{alg:quantize} can work channelwisely.
	
	\begin{enumerate}
		\item Instead of using floating point auxiliary weights for simulated
			  quantization \cite{n25_jacob2018quantization} or finding clever weight
			  initialization \cite{o_init_q}, we start by training the original float network, then calculate the optimal decimal
			  bits by minimizing the quantization error after a given number of steps $t_q$.
																																																																																																																																																																																																																															  
		\item When calculating the optimal decimal bits, instead of using the
			  standard mean square quantization error $\arg \min_{d} |\hat{x}_t - x_t|^2$,
			  we saturate $x_t$ to protect the quantization from outliers:
																																																																																																																																																																																																																															  
			  \begin{equation}
				  \begin{split}
					  d^* & = \arg \min_{d} |\hat{x}_t - \text{saturate}(x_t)|^2 \\
					  \text{saturate}(x) & = \text{clip}(x, \text{quantile}(x, s_l), \text{quantile}(x, s_u)) \\
					  \text{quantile}(x, a) & =  a\text{-th quantile of } x \\
					  s_l, s_u & \in [0, 1], s_l < s_u
				  \end{split}
				  \label{eq:qmse}
			  \end{equation}
																																																																																																																																																																																																																															  
			  Though being a simple modification, we show that it is critical for
			  applications like CycleGAN in Fig.~\ref{fig:cyclegan_demo} and Fig.~\ref{fig:feat_histogram}.  % fig:cyclegan_demo
																																																																																																																																																																																																																															  
		\item Similar to the Prune Operator in Alg.~\ref{alg:prune}, we also propose to
			  use a buffer to collect a short-term history of $x_t$ instead of only
			  relying $x_t$ for the optimization in Eq.~\ref{eq:qmse}.
	\end{enumerate}
	
	
	\begin{algorithm}[H]
		\SetAlgoLined
		\KwInput{number of bits $N$, quantize step $t_q$, saturation range $s_l,
		s_u$, buffer size $b_s$}     
		\KwOutput{decimal bits $d$}
		$B \gets $ empty queue with size $b_s$\\
		$d \gets 0$ \\
		\For{$t \gets 1$ to $T$}{
			append $x_t$ to B \\
			\eIf{$t < t_q$}{
				$o_t \gets x_t$	
				}{
				\If{$t\equiv t_q$}{$d \gets $ calculate from $B, s_l, s_u$ with Eq.~\ref{eq:qmse}}
				$o_t \gets  \text{clip}(\floor{x_t * 2^{d}}, -2^N, 2^N-1) / 2^d$
			}
		}
		\caption{Quantize Operator}
		\label{alg:quantize}
	\end{algorithm} 
	
	
	
	\subsection{Joint Pipeline}
	\label{sec:joint_pip}
	
	Although both prune and quantize operator work well independently, to unlock
	pruning and quantization on both weight and feature\footnote{To be precise, we
	quantize both feature and weight, while pruning either weight or feature.}, we
	design them to easily collaborate with each other through two dimensions,
	structurally and temporally. 
	
	
	Structurally, the key point is to apply pruning before quantization as indicated
	in Fig.~\ref{fig:pipeline}. \cite{n17_yu2020joint} has explained the benefit that
	pruning can help to reduce quantization error because 0 can always be perfectly
	quantized. 
	
	Temporally, we could jointly schedule by controlling the relationship between $t_0 +
	n\Delta t$ and $t_q$. Previous methods generally assume a Prune-then-Quantize
	paradigm without much scrutiny. However, we find this does not necessarily hold
	true when considering unstructured feature pruning and more applications. 
	
	\begin{itemize}
		\item  As shown in Sec.~\ref{sec:exp}, most experiments do demonstrate that
		it is better to Prune-then-Quantize temporally. However, in these cases, we
		find Quantize-then-Prune has a much worse performance on feature pruning
		scenario. It indicates a non-commutative property between quantization and pruning
		, which is not discussed by previous methods.
	
	
		\item In the super resolution experiment from Sec.~\ref{sec:exp_sr}, we find
		that Quantize-then-Prune actually brings much better performance than
		Prune-then-Quantize. Moreover, in addition to non-commutativity, quantization even
		improves feature pruning by a large margin, which is totally contrary to our intuition.
	\end{itemize}
	
	
	Though we don't fully explain these phenomena, we provide an insight through
	gradient perspective. 
	As shown in Fig.~\ref{fig:why_prune_then_quantize}, 
	we find that pruning will incur gradient peak when operating
	on feature, while straight-through gradient estimator tends to clamp the
	gradient by definition. It is likely this tension acts on the original gradients, causing
	these effects.
	
	\begin{figure}[h]
		\centering
		\includegraphics[width=0.7\linewidth]{plots/conv.pdf}
		\caption{An example of applying joint pruning and quantization on a
			convolution layer. Note the prune operator happens structurally before
			the quantize operator (but not necessarily temporally). We use dotted lines for prune operator since we
			apply it either on feature or weight.}
		\label{fig:pipeline}
	\end{figure}
	
	
	
	\section{Examples}
	
	We implement the Alg.~\ref{alg:prune} and Alg.~\ref{alg:quantize} in the form of
	two functions \texttt{quantize} and \texttt{prune} provided by our package
	\texttt{qsparse} that works seamlessly with pytorch built-in modules. In this
	section, we provide examples to demonstrate how simple and flexible they are for
	building joint pruned \& quantized networks \footnote{Detailed APIs and examples
		are provided in \href{https://todo.com}{https:/readthedocs.org/qsparse}}.
	
	
	
	\subsection{Feature Pruning \& Quantization}
	
	The following code creates a convolution layer whose output feature is
	pruned with $s_f = 0.5, t_0 = 1000, n = 3, \Delta t = 100$. 
	
	\begin{listing}[H]
		\python{snippets/prune_feat.py}
		\label{code:prune_feat}
	\end{listing}
	
	For the case of feature pruning \& quantization,  \texttt{quantize} and
	\texttt{prune} will just return normal pytorch modules which carries their own
	parameters. For the prune operator, the \mintinline{python}{'mask'} corresponds to
	$m_t$, the \mintinline{python}{'_cur_sparsity'} denotes $s_t$, and the
	\mintinline{python}{'_n_updates'} is an internal counter of the loop in line 4
	of Alg.~\ref{alg:prune}. For the quantize operator, the
	\mintinline{python}{'decimal'} represents $d$, \mintinline{python}{'bits'} is
	$N$, \mintinline{python}{'_quantized'} is a boolean variable for the check of
	line 8 in Alg.~\ref{alg:quantize}.
	
	% \begin{itemize}
	% 	\item For the prune operator, the \mintinline{python}{'mask'} corresponds to
	% 	      $m_t$, the \mintinline{python}{'_cur_sparsity'} denotes $s_t$, and the
	% 	      \mintinline{python}{'_n_updates'} is an internal counter of the loop in line 4
	% 	      of Alg.~\ref{alg:prune}.
																																																																																																																																																												
	% 	\item  For the quantize operator, the
	% 	      \mintinline{python}{'decimal'} represents $d$, \mintinline{python}{'bits'} is
	% 	      $N$, \mintinline{python}{'_quantized'} is a boolean variable for the check of
	% 	      line 8 in Alg.~\ref{alg:quantize}.
	% \end{itemize}
	
	
	\begin{listing}[H]
		\python{snippets/parameters_feat.py}
		\label{code:feat_parameters}
	\end{listing}
	
	
	
	\subsection{Weight Pruning \& Quantization}
	
	% briefly state our innovative approach
	% show how our approach works seamlessly with existing torch apis
	% how easy it is to access the mask/decimal points/bits
	% support directly resume from checkpoint without any problems
	
	The following code prunes the weight a convolution layer to 50\% with the given
	schedule.
	
	\begin{listing}[H]
		\python{snippets/prune_conv.py}
		% \caption{Weight Pruned Example}
		\label{code:prune_weight}
	\end{listing}
	
	Unlike existing libraries \cite{t_xilinx,QatTorch}, which provides
	a limited set of quantized layers separate from other
	pytorch modules, our library is agnostic to layer types can directly transform
	the \mintinline{python}{weight} attribute of the input layer into a pruned or
	quantized version during runtime. 
	
	This is to say, our library can works with any other pytorch modules, as long as
	their parameters can be accessed from the \mintinline{python}{weight} attribute,
	which aligns with pytorch convention. In the following, we show that by just
	chaining \mintinline{python}{quantize} and \mintinline{python}{prune} functions,
	we can obtain a quantized and pruned layer. 
	
	
	\begin{listing}[H]
		\python{snippets/prune_quantize_conv.py}
		% \caption{Weight Pruned \& Quantized Example}
		\label{code:prune_quantize_weight}
	\end{listing}
	
	
	The below snippet shows where the parameters are stored in a quantized and
	pruned layer, which indicates that it naturally supports to resume training from checkpoints.
	The original parameters (\texttt{weight, bias}) are left
	untouched. Users won't even need to change their weight initialization code
	when using this library. 
	
	
	
	\begin{listing}[H]
		\python{snippets/parameters.py}
		\label{code:weight_parameters}
	\end{listing}
	
	
	
	
	\section{Experiments}
	
	\label{sec:exp}
	
	To evaluate our method, we conduct experiments on five tasks: image
	classification, object detection, super resolution, image to image translation,
	and generative adversarial network. For each task, we apply 8bit quantization on
	both feature and weight of every layer, unstructured pruning with sparsity of
	50\% on either feature or weight except for the input \& output layer, if not
	specifically stated. In image classification, we also study the effect of timing
	to apply quantization and pruning during training. For a simpler notation, we
	use abbreviation to represent each experiment configuration as summarized in
	Table.~\ref{tb:abbr}.
	
	
	
	% To compare pruning on weight and feature, we keep all
	% hyper parameters the same between P(W) and P(F) except the target of pruning.
	
	
	\begin{table}[H]
		% \scriptsize
		\centering
		\begin{tabular}{|l|l|}
		\hline
		\textbf{Abbreviation} & \textbf{Description}                                                                           \\ \hline
		Q                     & Quantize all features and weights with 8 bits
		\\ \hline
		Q (Late) & Same as above, but quantization, or other operations indicated, happens near the end of training. \\ \hline
		P (W/F)               & P (W) means to prune 50\% weights, and P(F) means prune 50\% features.                         \\ \hline
		P-Q / Q-P             & P-Q means to apply pruning and then quantization
		temporally, Q-P means   the opposite.         \\ \hline
		BF    &  Buffer size in Alg.~\ref{alg:prune} and
		\ref{alg:quantize}, BF=1 means $b_s=1$. \\ \hline
		W Bits                & Bits for weight                                                                                \\ \hline
		F Bits                & Bits for feature map                                                                           \\ \hline
		W Sparsity            & Ratio of zeros in weight                                                                       \\ \hline
		F Sparisty            & Ratio of fixed zeros in feature map. These locations will be zero no   matter what inputs are. \\ \hline
		Reference/Ref      & Dense and floating point model. \\ \hline
		-- & Not applicable, e.g., F Sparsity will be `--' for methods don't
		apply feature pruning in Table~\ref{tb:cifar10_comp} \\ \hline
		\end{tabular}
	
		\caption{Description for experiment configuration abbreviations}
		\label{tb:abbr}
	\end{table}
	
	We implement each task by involving minimal code changes with our library
	on top of existing popular open-sourced repositories, which is also regarded as our
	reference and usually yields better accuracy than original papers. 
	We maintain hyper-parameters identical to the original settings except for 
	training epochs and when to apply quantization \& pruning. 
	We provide more details about experiment setups in
	appendix~\ref{apn:detailed_exp}. We release all experiment source codes as
	examples for our library\footnote{\href{http://todo.com}{https://github.com/mlzxy/qsparse/examples/}}.
	
	\subsection{Summary}
	
	In addition to verifying solid performance and robustness of our method, we discover many
	meaningful findings and summarize the major ones below.
	
	\begin{enumerate}
		\item Unstructured feature pruning demonstrates a completely different
		nature from the previous pruning paradigms.
		
		\begin{enumerate}
			\item It performs consistently worse than weight pruning under the same
			configuration.
			\item According to Fig.~\ref{fig:why_prune_then_quantize}, neural
			network exhibits a gradient
			peak behavior during pruning.
			\item 	It also shows a temporal dependency to
			quantization, as we discussed in Sec.~\ref{sec:joint_pip}. 
			\item Moreover, as we
			show in appendix~\ref{apn:more_exp}, it makes training unstable in some
			cases.
		\end{enumerate}
	
		However, given that it is clearly more beneficial for inference than the
		weight pruning counterpart from a matrix multiplication viewpoint. To the
		best of our knowledge, our method is the first one to propose unstructured
		feature pruning, and we believe that we uncover unstructured feature pruning
		as a practical scenario for model compression research.
		
	
		\item According to Fig.~\ref{fig:feat_histogram}, we find the feature value distribution
		of CycleGAN differs greatly from other networks. 
		\begin{enumerate}
			\item Though the distribution
			mostly concentrates around 0, it has a much longer tail which creates
			outliers for quantization.
			\item Furthermore, its feature carries more
			fine-grained information, which makes it necessary to use 12-bit
			quantization for feature in order to generate images with decent qualities.
		\end{enumerate}	
		It is still insufficient to claim these traits are universal for all generative
		models but it does shed some light on understanding the intrinsic difference
		between generative and discriminative networks.
		 
	\end{enumerate}
	
	
	\subsection{Image Classification}
	
	
	
	We conduct our image classification task on CIFAR10 \cite{o_cifar10}, which is
	commonly used for quantization and pruning evaluation. We apply quantization and
	pruning on MobileNetV2 \cite{mobilenetv2}, which is an already very lightweight
	network as shown in appendix~\ref{apn:benchmark}.
	The results are shown in Table~\ref{tb:cls_main}. We compare with previous
	methods in Table~\ref{tb:cifar10_comp}. 
	
	
	
	\textbf{Performance.} It can be seen that both prune and quantize operators work
	well independently and jointly for both feature and weight.  We basically have
	no accuracy loss in Q(Late) and P(W). Even in the case of both feature pruning
	and quantization, we only suffer a minor loss of less than 1. We argue our
	method stands strongly in performance against existing methods, but is far more
	versatile and practical\footnote{Note that it is
	inherently difficult to compare different quantization and pruning methods
	because of diversity and difference between configurations. We continue this discussion in
	appendix~\ref{apn:benchmark}.}.
	
	\begin{wrapfigure}[16]{r}{0.45\textwidth}
		\begin{center}
		  \scalebox{0.5}{
				\includegraphics{plots/pictures/grad_scale_analysis/why_sometime_quantize_is_position_sensitive/cifar.pdf}
			}
		\end{center}
		\caption{Visual explanation of why quantizing only works for CIFAR10 
		when applying during late stage of the training process.}
		\label{fig:why_quantize_later}
	  \end{wrapfigure}
	
	
	
	\textbf{Timing of quantization.} It is interesting to see that Q, Q-P(F) and
	Q-P(W) fail to converge completely, in which we quantize the network during the
	middle of the training. On the contrary, if we apply quantization near the end
	of training, e.g. Q(Late), the training sill converges. We find an explanation
	in Fig.~\ref{fig:why_quantize_later}. The gradient norm experiences a
	rise-and-fall during training, while straight through gradient estimator has a
	clamping effect on gradient. Therefore, larger gradient error will be introduced
	if quantization happens during the middle of training.
	
	Furthermore, the training results are well reflected in the summary 1.(a), 1.(c).
	
	\begin{table}[]
		\centering
		\begin{tabular}{rrrrrrrrrrr}
			\hline
					  Ref & Q  & P  (W) & P  (F) & P-Q (F) & P-Q (W) & Q-P
					 (F) & Q-P (W) & Q  (Late) & Q-P (F,Late) & Q-P (W,Late)  \\
			\hline
			 92.6      & 10 & 92.58  & 91.87  & 91.65   & 92.23   & 10      & 10     & 92.52     & 88.17         & 85.94     \\
			\hline
		\end{tabular}
		\caption{Validation accuracy with different prune \& quantization configurations on CIFAR10}
		\label{tb:cls_main}
	\end{table}
	
	
	\begin{table}[]
		\centering
		\begin{tabular}{@{}cccccccccl@{}}
			\toprule
			Method                                     & Network                                        & W Bits                    & F Bits                   & W Sparsity                   & F Sparsity                   & Reference Accuracy                     & \multicolumn{1}{c}{Accuracy}      \\ \midrule
			\multicolumn{1}{c|}{\cite{n2_yang2020automatic}}             & \multicolumn{1}{c|}{ResNet-20}                        & \multicolumn{1}{c|}{1.9}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{91.29}                 & 91.15 (-0.14)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n3_xiao2019autoprune}}                    & \multicolumn{1}{c|}{VGG-16}                       & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{79\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{93.4}                  & 91.5 (-1.9)                       \\ \midrule
			\multicolumn{1}{c|}{\cite{n4_van2020bayesian}}                    & \multicolumn{1}{c|}{VGG-7}                            & \multicolumn{1}{c|}{4.75} & \multicolumn{1}{c|}{5.4} & \multicolumn{1}{c|}{0\%}     & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{93.05}                 & 93.23 (+0.18)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n24_paupamah2020quantisation}}                   & \multicolumn{1}{c|}{MobileNet}                        & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{37.5\%}  & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{91.31}                 & 90.59 (-0.72)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{3}{*}{\cite{n29_liu2018rethinking}}}  & \multicolumn{1}{c|}{VGG-19}                           & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{80\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{93.5}                  & 93.52 (+0.02)                     \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{PreResNet-110}                    & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{95.04}                 & 95.06 (+0.02)                     \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{DenseNet-100}                  & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{95.24}                 & 95.21 (-0.03)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{2}{*}{\cite{n33_dettmers2019sparse}}}  & \multicolumn{1}{c|}{VGG16-C}                          & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{93.51}                 & 93 (-0.51)                        \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{WRN-22-8}                         & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{95.74}                 & 95.07 (-0.67)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n40_choi2016towards}}                   & \multicolumn{1}{c|}{ResNet-32}                        & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{77.8\%}  & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{92.58}                 & 92.64 (+0.06)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n41_choi2020universal}}                   & \multicolumn{1}{c|}{ResNet-32}                        & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{7.3\%}   & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{92.58}                 & 92.06 (-0.52)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n43_zhao2019variational}}                   & \multicolumn{1}{c|}{ResNet-20}                        & \multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{16.47\%} & \multicolumn{1}{c|}{16.47\%\footnote{It has a sparse feature
			because it applies structured pruning on weight, which corresponds to
			channel pruning on feature.}} & \multicolumn{1}{c|}{92.01}                 & 91.66 (-0.35)                     \\ \midrule
			\multicolumn{1}{c|}{\cite{n44_achterhold2018variational}}                   & \multicolumn{1}{c|}{DenseNet-76}                         & \multicolumn{1}{c|}{2}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}    & \multicolumn{1}{c|}{--}      & \multicolumn{1}{c|}{92.19}                 & 91.17 (-1.02)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{5}{*}{Ours}} & \multicolumn{1}{c|}{\multirow{5}{*}{MobileNetV2}}       & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{\multirow{5}{*}{92.6}} & \multicolumn{1}{c}{92.52 (-0.08)} \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{50\%}    & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.58 (-0.02)} \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{50\%}    & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.87 (-0.73)} \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{50\%}    & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.23 (-0.37)} \\
			\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}       & \multicolumn{1}{c|}{50\%}    & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.65 (-0.95)} \\ \bottomrule
		\end{tabular}
		\caption{Comparisons with previous pruning or quantization methods on CIFAR10}
		\label{tb:cifar10_comp}
	\end{table}
	
	
	
	
	
	  \subsection{Object Detection}
	  \label{sec:exp_detection}
	
	  We conduct our objection detection experiment on PASCAL VOC \cite{o_pascalvoc}
	  using Faster RCNN \cite{o_fasterrcnn} with a ImageNet \cite{o_imagenet}
	  pre-trained ResNet101 backbone. Since the original Faster RCNN trains on
	  images of different shapes each batch, it is impossible to obtain a fixed
	  unstructured pruning mask for convolution feature map as line 8 in
	  Alg.~\ref{alg:quantize}. Thus, we apply structured pruning on convolution features instead of
	  unstructured pruning. The results are shown in Table~\ref{tb:frcnn_main}. We
	  compare with previous methods in Table~\ref{tb:frcnn_comp}. 
	
	
	  \textbf{Performance.} It can be seen that we have the smallest performance
	  loss among other methods, even when weight \& feature are quantized and weight
	  are pruned 50\% (P-Q (W)). In the case of P-Q (F), we suffer a mAP drop of
	  1.47, but this is still smaller than that of
	  \cite{n28_krishnamoorthi2018quantizing, detect_he2017channel}.
	  
	 
	 
	  \textbf{Robustness.} Contrary to existing methods like
	  \cite{detect_li2019fully}, which introduces major overhauls over the object
	  detection network training procedures. Our method is less intrusive and works
	  without much modifications. Aligning with the original setting, we train with batch size equal to 1 and fix all
	  pre-trained batch normalization layers. Note that we do not prune or quantize for the first 5
	  residual blocks because they are frozen originally and unfreezing
	  will collapse the training even for reference network. However, this
	  limitation can be easily discarded as long as group normalization or synchronized
	  batch normalization according to \cite{he2019rethinking}. Thus, we do not
	  regard this as our limitation.
	
	  \textbf{Effect of Buffer Size.} From Table~\ref{tb:frcnn_main}, we can see that
	  the mAP will drop 0.4 from P-Q (F) if we set $b_s$ to 1, which indicates that
	  decimal bits $d$ and pruning mask $m$ can be more accurately computed from
	  multiple batches especially when original batch size is small. 
	
	  Furthermore, the training results are well reckoned in the summary 1.(a), 1.(c).
	
	
	  
	  \begin{table}[]
		  \centering
		  \begin{tabular}{lrrrrrrrrr}
			  \hline
				  & Reference & Q  & P  (W) & P  (F) & P-Q (F) & P-Q (F, BF=1) & P-Q (W) & Q-P (F) & Q-P (W) \\
			  \hline
			  MAP & 74.47    & 74.25    & 74.33 & 73.04 & 73  & 72.6   & 74.44  & 70.13  & 74.13  \\
			  \hline
		  \end{tabular}
		  \caption{Faster RCNN results with different prune \& quantization configurations on PASCAL VOC 2007 test set.}
		  \label{tb:frcnn_main}
	  \end{table}
	  
	  
	  \begin{table}[]
		  \centering
		  \begin{tabular}{@{}cccccccc@{}}
			  \toprule
			  Method                                  & Detection Framework          & W Bits & F Bits & W Sparsity & F Sparsity & Reference mAP          & mAP           \\ \midrule
			  \cite{n27_yang2019quantization}         & YOLO-v2                      & 8      & 8      & --         & --         & 72.64                  & 72.5 (-0.14)  \\ \midrule
			  \cite{n28_krishnamoorthi2018quantizing} & SSD
			  & 7      & 8      & --         & --         & 77.8                   &
			  76.1 (-1.7)   \\ \midrule
			  \cite{detect_he2017channel}  & Faster RCNN & -- & -- & --  & 50\% & 68.7
			  & 66.9 (-1.8) \\ \midrule
			  \cite{detect_wei2018quantization}  & Faster RCNN & 8 & 8 & --  & -- &
			  44.6	  & 47.0 (+2.4) \\ \midrule
			  \cite{detect_yin2016quantization}  & R-FCN & 6 & -- & --  & -- & 78.94
			  & 78.24 (-0.7) \\ \midrule
			  \multirow{3}{*}{Ours}                   & \multirow{3}{*}{Faster RCNN} & 8      & 8      & --         & --         & \multirow{3}{*}{74.47} & 74.25 (-0.22) \\
													  &                              & 8      & 8      & 50\%       & --         &                        & 74.44 (-0.03) \\
													  &                              & 8      & 8      & --         & 50\%       &                        & 73 (-1.47)    \\ \bottomrule
		  \end{tabular}
		  \caption{Comparisons with previous pruning or quantization methods on PASCAL VOC 2007}
		  \label{tb:frcnn_comp}
	  \end{table}
	  
	
	\subsection{Super Resolution}
	
	\label{sec:exp_sr}
	
	We conduct our super resolution task on 91-image \cite{o_91image} (training set)
	and Set5 \cite{o_set5} (validation set) with efficient sub-pixel convolution
	network (ESPCN) \cite{espcn}, which is a 3-layer convolution network without
	normalization layer. Note that we find the training is not stable enough.
	Therefore, for each configuration, we run five times and peak the best model, and
	the results are shown in Table~\ref{tb:sr_main}. 
	
	\textbf{Performance.} In Table~\ref{tb:sr_main}, though every configuration
	suffers a performance drop, our results still have better PSNR than the
	original result reported in \cite{espcn} except for those feature pruning cases.
	
	\textbf{Quantize helps Feature Pruning.} In this case, not only we find that it
	is more beneficial to quantize first and then prune, we also observe that
	feature pruning yields better performance with quantization. It indicates that
	the non-trivial relationship between quantization and feature pruning as we
	discussed in Sec.~\ref{sec:joint_pip}. This corresponds to summary 1.(c).
	
	\textbf{Gradient Peak.} In Fig.~\ref{fig:why_prune_then_quantize}, we show that
	feature pruning will incur gradient peaks. It is intuitive from hindsight since
	the network is trying to learn more by having large gradients when fractions of
	features suddenly become zero. This corresponds to summary 1.(b). 
	
	\begin{table}[]
		\footnotesize
		\centering
		\begin{tabular}{rrrrrrrrrr}
			\hline
			Ref & Q       & P  (W)  & P  (F)  & P-Q (W) & P-Q (F) & Q-P (W) & Q-P (F) \\
			
			\hline
			32.86 & 32.69 & 32.77 &  31.52  & 32.57 & 31.7 & 32.59 & 32.12   \\
			\hline
		\end{tabular}
		\caption{PSNR (peek signal-to-noise ratio) with different prune \& quantization configurations on Set5}
		\label{tb:sr_main}
	\end{table}
	
	
	
	
	\begin{figure}[]
		\centering
		\begin{minipage}{.5\textwidth}
			\centering
			\scalebox{0.5}{
				\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_feat.pdf}
			}
		\end{minipage}%
		\begin{minipage}{.5\textwidth}
			\centering
			\scalebox{0.5}{
				\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_grad.pdf}
			}
		\end{minipage}
																													
		\caption{Visual demonstration of gradient peak during feature pruning. Gradients are sampled from feature map instead of weight.}
		\label{fig:why_prune_then_quantize}
	\end{figure}
	
	
	
	
	
	
	
	
	
	\subsection{Image to Image Translation and Generative Adversarial Network}
	
	We conduct our image to image translation task on facades dataset with Pix2Pix
	network \cite{pix2pix}, and our GAN task on horse2zebra dataset with CycleGAN
	\cite{o_cyclegan}. Both of them applies an encoder-decoder structured network,
	while the Pix2Pix uses UNet \cite{unet} and CycleGAN uses a variant of ResNet
	with deconvolution layers. In Fig.~\ref{fig:pix2pix_demo} and
	\ref{fig:cyclegan_demo}, we demonstrate some generated samples, and we provide
	more samples in appendix~\ref{apn:more_demos}.
	
	\textbf{Performance.} From Fig.~\ref{fig:pix2pix_demo}, it is hard to
	distinguish the quality difference between the reference and quantized only
	network, despite some color difference. If we add weight pruning, we can observe
	some details get blurry. However, if we prune feature, though the overall
	structure remains, the color becomes unnatural and some major distortions could
	be spotted. From Fig.~\ref{fig:cyclegan_demo}, we can find that weight pruned
	network transfers the texture correct but the color transfer seems unfinished,
	while the feature pruned network looks like the opposite, which may represent a
	division of functions within the network. 
	
	\textbf{Feature Distribution and Information Granularity.} From
	Fig.~\ref{fig:feat_histogram} and \ref{fig:cyclegan_demo} about CycleGAN, we are
	amazed to discover that its feature distribution has a much longer tail, and its
	generative quality is very sensitive to minor changes in feature, which
	corresponds to to summary 2.
	
	\begin{figure}[]
		\begin{minipage}[t]{0.48\linewidth}
			\scalebox{0.28}{
			\includegraphics{plots/pictures/pix2pix/main33/24.pdf}
		}
		\caption{Examples of generated images from Pix2Pix networks with different
		configurations. }
		\label{fig:pix2pix_demo}
		\end{minipage}%
			\hfill%
		\begin{minipage}[t]{0.48\linewidth}
			\scalebox{0.28}{
			\inputpgf{plots/pictures/cyclegan/main}{3.pgf}
		}
		\caption{Examples of generated images from CycleGAN networks with different
			configurations. 
			It is clear to see the saturated quantization works as an important factor,
		and more than 8 bits are required for this generative task.}
		\label{fig:cyclegan_demo}
		\end{minipage} 
		\end{figure}
	
	
	
	
	
	\begin{figure}[]
		\centering
		\begin{minipage}{.5\textwidth}
			\centering
			\scalebox{0.5}{
				\includegraphics{plots/pictures/feat_histogram_analysis/sr.pdf}
			}
		\end{minipage}%
		\begin{minipage}{.5\textwidth}
			\centering
			\scalebox{0.5}{
				\includegraphics{plots/pictures/feat_histogram_analysis/cycle.pdf}
			}
		\end{minipage}
		\caption{Feature histogram comparison between the network of super
			resolution and CycleGAN. It is obvious to see that the features of
			CycleGAN are much more long-tailed, which our saturated quantization can
			handle well. }
		% 	Note that it is also natural to consider logarithmic
		% 	quantization for long-tailed distribution \cite{o_hubara2017quantized},
		% but it may result in additional difficulty for inference acceleration.
		\label{fig:feat_histogram}
	\end{figure}
	
	
	
	
	\section{Conclusion}
	
	In this paper, we design a joint quantization and pruning methods, uncover
	unstructured feature pruning as an important scenario for model compression
	research and release our method as a software package. Moreover, we conduct
	thorough experiments on a wide range of tasks and discover many interesting
	findings.
	
	Admittedly, this work bears its own limitations. We still could not fully
	explain the complex inter-dependency between feature pruning and quantization,
	and feature distribution of generative adversarial networks. Feature pruning
	still suffers from non-negligible performance drop. However, we believe these
	limitations could be regarded as future possibilities. It will be interesting to
	see what could be built upon our findings.
	

==> include.backup0922/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[strings]{underscore}
% \usepackage{url}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{bbold}
\usepackage{graphicx}
\usepackage{fancybox}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage[noend,algoruled,linesnumbered, rightnl]{algorithm2e}
\usepackage{seqsplit}
\usepackage{multirow}
\usepackage{float}
\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{caption}
\usepackage{minted}
\usepackage{subcaption}

\newtheorem{theorem}{Theorem}

\renewcommand{\url}[1]{\texttt{\seqsplit{#1}}}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand\tocite[1]{\textcolor{blue}{[#1]}}
\newcommand{\comment}[1]{}
\long\def\/*#1*/{}

\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


\newcommand{\python}[1]{
\inputminted[
frame=single,framesep=10pt,
bgcolor=lightergray,
fontsize=\footnotesize,
]{python}{#1}
}
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\SetKwInput{KwInput}{Input} % just a guess
\SetKwInput{KwOutput}{Output} % just a guess
\definecolor{lightergray}{RGB}{242, 242, 242}

\newcommand{\bsquare}{{\scriptsize $\blacksquare$}}
\newcommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\let\includegraphicsWithoutPath\includegraphics
\renewcommand{\includegraphics}[2][]{\includegraphicsWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}


==> include.backup0926/author.tex <==
\title{Quantized Sparse: Joint Quantization and Pruning Training in Python}


\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@ucsd.edu}
	\And
	Ian Colbert\\
	UC San Diego\\
	\texttt{icolbert@ucsd.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@ucsd.edu} \\
	\And
	Srinjoy Das\\
	UC San Diego\\
	\texttt{s2das@ucsd.edu} 
}

\hypersetup{
pdftitle={Quantized Sparse: Joint Quantization and Pruning Training in Python},
pdfsubject={deep learning},
pdfauthor={Xinyu Zhang},
pdfkeywords={Quantization, Neural Networks, Pruning, Software Tool, Python, Pytorch, Model
Compression, Object Detection, Super Resolution, Classification, Image to Image
Translation, Generative Adversarial Network, CycleGAN},
}

==> include.backup0926/body.tex <==

\begin{abstract}
					
	In this paper, we propose a joint quantization and pruning method on both
	feature and weight. With our method, we study unstructured feature pruning extensively and
	uncover it to be an important yet overlooked problem for model compression
	research. We verify our method to have strong performance and robustness through
	experiments on image classification, object detection, super resolution, image
	to image translation, and generative adversarial network. Furthermore, we
	release our method as a pytorch-based python package at
	\ourlib, which is surprisingly
	simple and flexible to accommodate various use cases.
						
\end{abstract}
	
	
	
\section{Introduction}
	
Deep neural networks have been widely deployed in various applications. To
improve the neural network inference efficiency, quantization and pruning
have become the indispensible procedures before the deployment of a network
model. The former reduces the bit-width of weight and feature, which
provides smaller memory footprint and fixed-point arithmetic acceleration.
The latter pruning weight or neurons to produce a sparse network which
requires less memory and computation budget. As we can see in
Sec.~\ref{sec:relate} and appendix~\ref{apn:related_work}, there have been a
great deal of research work in these two directions.
	
Despite many successes, we believe that the current study still have remaining
problems to solve.  
	
\begin{itemize}
	\item[\bsquare] Pruning and quantization are often considered to be able to solve
	      independently \citep{n21_liang2021pruning, o_paupamah2020quantisation},
	      though there have been some recent research to study both quantization and
	      pruning in a unified scope.
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item[\bsquare] Not enough attention has been paid to unstructured
	      pruning on the feature map. Although there are many studies on
	      unstructured and structured weight pruning, we
	      argue that it is far more beneficial for inference if we apply
	      unstructured pruning on feature rather than weight. Take
	      convolution as an example, we can save an entire dot
	      product by only skipping a single output feature value \citep{convarith_dumoulin2016guide}.
	      	      	      	      	      			  
	      %   \citep{h_gemm}
	      %   \citep{h_colbert2021energy,h_jha120data}
	      % \citep{detect_li2019fully}
	      %   \citep{detect_tzelepis2019deep} \citep{detect_wei2018quantization}																																																																																																																																																																																																								  
	\item[\bsquare] Most existing work are focused on classification tasks, and some work have covered
	      object detection \citep{detect_li2019fully}.
	      However, there is still very little pruning and quantization
	      research on generative tasks like generative adversarial networks
	      (GAN) or image to image translation.
	      	      	      	      	      
	      	      	      	      	      																																																																																																																																																																																																																																   
	\item[\bsquare] None of available network compression tools can provide both a
	      set of flexible APIs and joint quantization \& pruning training capability,
	      despite the large number of publications on related directions.
	      	      	      	      	      																																																																																																																																																																																																																																   
\end{itemize}
	
	
Therefore, to solve the above problems, we make the following contributions in
this paper. 
	
\begin{enumerate}
	\item We propose a joint quantization and pruning method, and points out
	      that these two operations are non-commutative and even dependant,
	      instead of independent in certain cases.
	      	      	      	      	      																																																																																																																																																																																																																																  
	      	      	      	      	      	
	\item To the best of our knowledge, this is the first work that studies
	      unstructured feature pruning extensively. We discover it works in a
	      completely different pattern to existing pruning paradigm, which identifies
	      it to be a new and important scenario for model compression
	      research. 
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item We verify our method to have strong performance and robustness on
	      image classification, object detection, super resolution, Pix2Pix
	      \cite{pix2pix} and CycleGAN \citep{o_cyclegan}, where we also
	      discover and summarize many meaningful findings, especially from
	      generative tasks.
	      	      	      	      	      																																																																																																																																																																																																																															  
	\item We release our method as a pytorch-based python package.
	      Contrary to existing libraries like \citep{t_xilinx}, which only
	      provides a limited set of 
	      quantized or pruned modules isolated from other toolchain, 
	      we come up with an entirely innovative design.
	      Our library only exposes two layer-level primitives and works
	      seamlessly with any other pytorch modules.
	      											  
	      											 
	      %   which is
	      %   surprisingly simple by only exposing two layer-level primitives for
	      %   quantization and pruning, and could be easily extended and integrated
	      %   with other use cases.
\end{enumerate}
					
					
					
					
\section{Related Works} 
\label{sec:relate}
				
Due to space limit and the fact that both quantization and pruning are large areas of research
with broad practical impacts, we will only outline concepts and work closely related to our contributions
in this section. We provide a much broader and detailed review in appendix~\ref{apn:related_work}.
				
				
					
\textbf{Quantization.} Quantization \citep{n16_wu2020integer} is the process
of quantifying floating numbers with integer equivalents and can be applied
on both weights and feature. Post-training quantization
\citep{n26_lee2018quantization} aims on converting a trained float network
to quantized version without adequate access to training data, which is
convenient but sometimes suffers from accuracy degradation.
Quantization-aware training \citep{o_hubara2017quantized} involves
quantization into the training process, which usually provides better
accuracy but requires more efforts. Most work are focused on classification
tasks, while there are some recent work \citep{detect_wei2018quantization,
detect_li2019fully} on quantization for objection detection networks.
\citep{n23_wang2019qgan} quantizes the weight of a GAN to low bit-width on
CIFAR10 and CelebA \citep{o_celebA}.
					
				
					
					
\textbf{Pruning.} Sparsity is a long-standing research problem in the neural
network domain \citep{n38_gale2019state, n35_hoefler2021sparsity}, and
pruning is an important technique to obtain sparse neural network by
removing unimportant connections. Finetuning-based methods prune gradually
during training \citep{n45_zhu2017prune}, and retraining-based methods
retrain networks with pruned structure \citep{n37_frankle2018lottery}. There
have been debates about which one is better \citep{n29_liu2018rethinking,
renda2020comparing}. Most of known pruning methods act on weight, and can be
categorized as structured \citep{o_liu2017learning} and unstructured pruning
\citep{o_han2015learning}, while the former one requires to removes a
channel of weight together and the latter one can remove weight arbitrarily.
Most work are focused on classification tasks, and
\citep{detect_he2017channel} proposes a layer-wise structured pruning method
for object detection. There are some work connects GAN with sparsity
\citep{n34_zhou2020sparse}, but their major focus is on how to use sparse
regularization to improve generative quality instead of pruning.
				
				
					
\textbf{Joint Quantization and Pruning.} There are relatively few work that jointly
consider pruning and quantization. Most work assumes a Prune-then-Quantize
pipeline \citep{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint}. 
\citep{n21_liang2021pruning,
n24_paupamah2020quantisation} further claim that pruning and quantization can
be studied independently. 
					
				
					
					
\textbf{Neural Network Compression Toolbox.} There are many open-source
model compression tools that provide pruning or quantization functionality.
However, as far as our best knowledge, none of them offer joint pruning \&
quantization. Moreover, many tools are designed to be heavily inflexible and
some even requires developers to write code in a domain-specific language
(DSL). We discuss this more details in appendix~\ref{apn:related_work}.
					
					
				
					
					
					
\section{Method}
\label{sec:method}
			
Our method has three modules. We explain our pruning and quantization
operators design in Sec.~\ref{sec:quantize_operator} and
\ref{sec:prune_operator}, and a joint pipeline
to collaborate them in structural and temporal dimensions in Sec.~\ref{sec:joint_pip}. We also explain
why not to adopt a commonly used Prune-then-Quantize pattern and how
unstructured feature pruning works.
					
% Our approach consists of three modules. The first two are pruning and
% quantization operators. We design them to be able to work
% independently on both feature and weight. Then we propose a joint pipeline that
% allows two operators to collaborate smoothly.
					
\subsection{Quantization Operator}
\label{sec:quantize_operator}	
			
% algorithm block
% supports channelwise, when apply either on feature/weight can channelwise
					
Our quantization operator is an improved version from
\citep{o_hubara2017quantized}, by which they both leverage "straight-through
estimator" for gradient calculation and follow a inference-friendly linear
quantization scheme \citep{n25_jacob2018quantization}. Giving input $x_t$ to
denote either weight or feature at step $t$, $N$ be the total number of
bits, $d$ be the number of decimal bits\footnote{Bits used to represent
	fractions}, the quantized $x_t$ can be represented by $\hat{x}_t$:
					
					
\begin{equation}
	\begin{split}
		\hat{x}_t & = \text{clip}(\floor{x_t * 2^{d}}, -2^N, 2^N-1) / 2^d \\
		\frac{\partial Loss}{\partial x_t} & = \text{clip}(\frac{\partial Loss}{\partial \hat{x}_t}, -2^{N-d}, 2^{N-d} - 1)
	\end{split}
	\label{eq:quantize}
\end{equation}
					
					
However, we make two simple yet effective enhancements on top of existing methods, as
explained below and Alg.~\ref{alg:quantize}. 
			
% Note we also adopt the per-channel
% quantization scheme from \citep{n28_krishnamoorthi2018quantizing}, thus the
% Alg.~\ref{alg:quantize} can work channelwisely.
					
\begin{enumerate}
	\item \textbf{Delayed Quantization Error Minimization.} Instead of using floating point auxiliary weights for simulated
	      quantization \citep{n25_jacob2018quantization} or finding clever weight
	      initialization \citep{o_init_q}, we start by training the original float network, then calculate the optimal decimal
	      bits by minimizing the quantization error after a given number of
	      steps $t_q$. By thorough experiments in Sec.~\ref{sec:exp}, we
	      shall that it makes our method robust enough
	      to accommodate initialization and training dynamics of various applications.
	      		      		      		      		      																																																																																																																																																																																																																															  
	\item \textbf{Saturated Quantization.} When calculating the optimal decimal bits, instead of using the
	      standard mean square quantization error $\arg \min_{d} |\hat{x}_t - x_t|^2$,
	      we saturate $x_t$ to protect the quantization from outliers:
	      		      		      		      		      																																																																																																																																																																																																																															  
	      \begin{equation}
	      	\begin{split}
	      		d^* & = \arg \min_{d} |\hat{x}_t - \text{saturate}(x_t)|^2 \\
	      		\text{saturate}(x) & = \text{clip}(x, \text{quantile}(x, s_l), \text{quantile}(x, s_u)) \\
	      		\text{quantile}(x, a) & =  a\text{-th quantile of } x \\
	      		s_l, s_u & \in [0, 1], s_l < s_u
	      	\end{split}
	      	\label{eq:qmse}
	      \end{equation}
	      		      		      		      		      																																																																																																																																																																																																																															  
	      Later we show that it is critical for
	      applications like CycleGAN in Fig.~\ref{fig:cyclegan_demo} and Fig.~\ref{fig:feat_histogram}.  % fig:cyclegan_demo
	      		      		      		      		      																																																																																																																																																																																																																															  
	      % \item Similar to the Prune Operator in Alg.~\ref{alg:prune}, we also propose to
	      %       use a buffer to collect a short-term history of $x_t$ instead of only
	      %       relying $x_t$ for the optimization in Eq.~\ref{eq:qmse}.
\end{enumerate}
					
			
				
\subsection{Pruning Operator}
\label{sec:prune_operator}
					
					
Our pruning operator is an improved version from \citep{n45_zhu2017prune}.
Specifically, it is an automated gradual pruning algorithm where the
sparsity is increased during training for $n$ repetitions till the final
sparsity $s_f$. Let $\Delta t$ be the interval between each pruning step,
$t_0$ be the start step of the pruning procedure, the sparsity at time $t$
is denoted by $s_t$ in Eq.~\ref{eq:sparsity}.
					
\begin{equation}
	s_{t}=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta t}\Bigr\rfloor\right)^{3} \right) 
	\label{eq:sparsity}
\end{equation}
					
At each pruning step when $t = t_0 + i \Delta t, i\in [n]$, a mask $m_t$ is
calculated by zeroing out the smallest magnitude input until the $s_t$ is
reached. This mask will be kept the same for both training and inference until
the next pruning step if exists. 
					
The modification we make is instead of only depending on magnitude of the
current input, we maintain an input buffer so we construct the mask from the
magnitude of a history of inputs. Later we see that the input buffer is important for
unstructured feature pruning in Table~\ref{tb:frcnn_main}. 
					
						
\begin{multicols}{2}
	\begin{minipage}{0.49\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\SetNlSkip{0em}
			\KwInput{number of bits $N$, quantize step $t_q$ \\ \hspace{2em} saturation range $s_l,
			s_u$}     % , buffer size $b_s$
			\KwOutput{decimal bits $d$}
			% $B \gets $ empty queue with size $b_s$\\
			$d \gets 0$ \\
			\For{$t \gets 1$ to $T$}{
				\eIf{$t < t_q$}{
					$o_t \gets x_t$	
					}{
					\If{$t\equiv t_q$}{$d \gets $ calculate from $x_t, s_l, s_u$ with Eq.~\ref{eq:qmse}}
					$o_t \gets \text{clip}(\floor{x_t * 2^{d}},$ \\
					\hspace{4em} $-2^N, 2^N-1) / 2^d$
				}
			}
			\caption{Quantize Operator}
			\label{alg:quantize}
		\end{algorithm} 
	\end{minipage}
									
	\begin{minipage}{0.49\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\KwInput{sparsity $s_f$, start step $t_0$, interval $\Delta t$ \\
				\hspace{3em} repetition $n$, buffer size $b_s$}     
			\KwOutput{mask $m_T$}
																																																																																																													
			$B \gets $ empty queue with size $b_s$\\
			$s_0 \gets 0$ and $m_0 \gets \mathbb{1}$ \\
			\For{$t \gets 1$ to $T$}{
				append $x_t$ to B \\
				$s_{t}=s_{f} \Big(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta
					t}\Bigr\rfloor\right)^{3} \Big)$ \\
				\eIf{$s_{t-1} \neq s_t$}{
					$m_t \gets $ calculate mask from $B$ and $s_t$
					}{
					$m_t \gets m_{t-1}$
				} 
				$o_t \gets x_t * m_t$
			}
			\caption{Pruning Operator}
			\label{alg:prune}
		\end{algorithm} 
	\end{minipage}
									
\end{multicols}
					
				
					 
Giving input $x_t$ to denote either weight or feature at step $t$, $T$ as
the total number of steps, $o_t$ to denote the operator output, the pruning
operator mechanism is demonstrated in Alg.~\ref{alg:prune}. The mask
calculation in line 8 will find the positions with smallest magnitude
averaged over a buffer of history inputs.
					
				
					
					
\subsection{Joint Pipeline}
\label{sec:joint_pip}
					
Both prune and quantize operator can work independently on either weight or
feature, it's natural to design a
jointly pruned and quantized layer as shown in Fig.~\ref{fig:pipeline},
where pruning is applied before quantization structurally as
\citep{n17_yu2020joint} has explained the benefit that pruning can help to
reduce quantization error because 0 can always be perfectly quantized. 
However, we point out two previously under-studied perspectives, temporal
collaboration between two operators and unstructured feature pruning.
			
\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\linewidth]{plots/conv.pdf}
	\caption{An example of applying joint pruning and quantization on a
		convolution layer. We use dotted lines for prune operator since it
	is applied either on feature or weight.}
	\label{fig:pipeline}
\end{figure}
			

\subsubsection{Unstructured Feature Pruning}
		
Due to the flexibility of our method, we find it is possible to apply the
prune operator in Alg.~\ref{alg:prune} directly on feature map, which we
call \textit{unstructured feature pruning}. Similar to weight pruning, it
will generate a fixed binary mask for each feature, and masked feature
values will always be zero. To put in an intuitive way of speaking, it is
like having \q{holes} on designated locations of a feature map.

In many ways, unstructured feature pruning is a worthy problem. On the one
hand, unstructured feature pruning is more flexible than structured pruning
\footnote{Structured pruning is equivalent to weight and feature because it
operates per channel.} because it does not have to prune at a per-channel
granularity. On the other hand, unstructured feature pruning can be much
more rewarding for inference than unstructured weight pruning because
skipping a single output value could save an entire dot product.


			
			
\subsubsection{Temporal Collaboration}
					
Temporally, we could jointly schedule two operators by controlling the
relationship between $t_0 + n\Delta t$ in Alg.~\ref{alg:prune} and $t_q$ in
Alg.~\ref{alg:quantize}. Previous methods generally assume a
Prune-then-Quantize paradigm ($t_0 + n\Delta t > t_q$) without much
scrutiny. However, we find this argument is not sufficient to encompass the
relationship between pruning and quantization when taking unstructured
feature pruning into consideration. 
					
\begin{itemize}
	\item \textbf{Non-Commutativity.} Although many experiments in Sec.~\ref{sec:exp} demonstrate that
	      Prune-then-Quantize temporally provides a better accuracy. 
	      However, in these cases, we find Quantize-then-Prune has a much
	      worse performance on feature pruning scenario. It indicates a
	      non-commutative property between quantization and pruning, which
	      is not discussed by previous methods.
	      		      		      		      		      	
	      		      		      		      		      	
	\item \textbf{Quantize-Then-Prune.} In Sec.~\ref{sec:exp_sr}, we find a reversed relationship where
	      Quantize-then-Prune actually brings much better performance.
	      
	      %   Prune-then-Quantize almost fails to converge. 
	      			 
	      %   Moreover, in addition to non-commutativity, quantization even
	      %   improves feature pruning by a large margin, which is totally
	      %   contrary to our intuition.
	\item \textbf{Quantize-Help-Prune.} In Sec.~\ref{sec:exp_sr}, we even
	      observe that quantization is critical for feature pruning, and feature
	      pruning alone almost fails to converge.
\end{itemize}
					
\textbf{Gradient Peak Effect.} Furthermore, we provide a gradient
perspective to explain these phenomena. As shown in
Fig.~\ref{fig:why_prune_then_quantize}, we find that pruning will incur
spikes on gradient of activations when operating on feature because loss
will be more concentrated on the remaining values. We suppose this could
even be exacerbated through back-propagation. Moreover, the gradient peak
could correlate with two additional dynamics: (1) the gradient clamping from
straight-through gradient estimator in Eq.~\ref{eq:quantize}. (2) gradient
of the origin model. We could obtain various training results when
the tension among these dynamics goes differently. 
	
Therefore, we show that unstructured feature pruning works in a
completely different pattern to existing pruning paradigms, which we believe
could identify it to be a practical scenario for model compression research.
Based on our findings, we propose pruning and quantization to collaborate
temporally but not in a pre-defined manner.
	


\section{Software Interface}
					

We release our method in a pytorch-based software package. In
Listing~\ref{code:interface}, we demonstrate how simple and flexible it can
make for pruned and quantized training. Unlike existing libraries
\citep{t_xilinx,QatTorch}, we propose a novel design which directly
transforms the weight attribute of the input layer into a pruned or
quantized version during runtime. This is to say, our library is
layer-agnostic and can work with any pytorch modules, as long as their
parameters can be accessed from the weight attribute. Additionally, it
leaves the original weight and bias untouched. Users won't even need to
change weight initialization code for pruned and quantized training.
More information can be found at \ourlib.


					
\begin{listing}[]
	\python{snippets/interface.py}
	\vspace{-2.5em}
	\caption{Examples to demonstrate our software interface for quantization and pruning}
	\label{code:interface}
\end{listing}
					
					
					
\section{Experiments}
					
\label{sec:exp}
					
To evaluate our method, we conduct experiments on five tasks: image
classification, object detection, super resolution, image to image translation,
and generative adversarial network. 
	
For each task, if not specifically stated, we apply 8-bit quantization on
both feature and weight of every layer, unstructured pruning with sparsity
of 50\% on either feature or weight except for the first \& last layer.
For a simpler notation, we use abbreviation to represent each experiment
configuration as summarized in Table.~\ref{tb:abbr}.
					
					
\begin{table}[H]
	% \scriptsize
	\centering
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Abbreviation} & \textbf{Description}                                                   \\ \hline
		Q                     & Quantize all features and weights with 8 bits                          
		\\ \hline
		P (W/F)               & P (W) means to prune 50\% weights, and P(F) means prune 50\% features. \\ \hline
		P-Q / Q-P             & P-Q means to apply pruning and then quantization                       
		temporally, Q-P means   the opposite.         \\ \hline
		BF                    & Buffer size in Alg.~\ref{alg:prune}, BF=1 means $b_s=1$.               \\ \hline
		W/F Bits              & Bits for weight or feature                                             \\ \hline
		W/F Sparsity          & Ratio of fixed zeros in weight or feature map                          \\ \hline
		Reference/Ref         & Dense and floating point model.                                        \\ \hline
		--                    & Not applicable, e.g., F Sparsity will be `--' for methods don't        
		apply feature pruning. \\ \hline
	\end{tabular}
										
	\caption{Description for experiment configuration abbreviations}
	\label{tb:abbr}
\end{table}
					
We implement each task by applying minimal code changes with our library
on top of existing popular open-source implementations. 
We maintain most hyper-parameters identical to the original settings except for 
training epochs and when to apply quantization \& pruning. 
We provide more details about experiment setups in
appendix~\ref{apn:detailed_exp}. We release all experiment source code as
examples for our library.
					
					
					
\subsection{Image Classification}
					
					
We conduct our image classification task on CIFAR10 \citep{o_cifar10} with
MobileNetV2 \citep{mobilenetv2}, Results of different configurations are shown
in Table~\ref{tb:cls_main}. We compare with previous methods in
Table~\ref{tb:cifar10_comp}. We basically have no accuracy loss in Q and P(W).
Even in the case of both feature pruning and quantization, we only suffer a
minor loss of less than 1.
					

\begin{table}[]
	\centering
	% \vspace{-0.5em}
	\begin{tabular}{rrrrrrrrrrr}
		\hline
		& Ref & Q  & P  (W) & P  (F) & P-Q (F) & P-Q (W) & Q-P
		(F) & Q-P (W)   \\
		\hline
		Accuracy & 92.6 & 92.52 & 92.58 & 91.87 & 91.65 & 92.23 & 88.17 & 85.94  \\
		\hline
	\end{tabular}
	\caption{Validation accuracy with different prune \& quantization
	configurations on CIFAR10. Q-P performs
	much worse than P-Q, which indicates a non-commutative
	property between quantization and pruning. }
	\label{tb:cls_main}
	\vspace{-1.5em}
\end{table}
	
				
					
\begin{table}[]
	\centering
	\vspace{-1em}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccccccl}
			\toprule
			Method                                                                        & Network                                           & W Bits                    & F Bits                   & W Sparsity                  & F Sparsity                & Ref Accuracy                               & \multicolumn{1}{c}{Accuracy}      \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n2_yang2020automatic}}}                    & \multicolumn{1}{c|}{ResNet-20}                    & \multicolumn{1}{c|}{1.9}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{91.29}                 & 91.15 (-0.14)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n3_xiao2019autoprune}}}                    & \multicolumn{1}{c|}{VGG-16}                       & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{79\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.4}                  & 91.5 (-1.9)                       \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n4_van2020bayesian}} }                     & \multicolumn{1}{c|}{VGG-7}                        & \multicolumn{1}{c|}{4.75} & \multicolumn{1}{c|}{5.4} & \multicolumn{1}{c|}{0\%}    & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.05}                 & 93.23 (+0.18)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n24_paupamah2020quantisation}}}            & \multicolumn{1}{c|}{MobileNet}                    & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{37.5\%} & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{91.31}                 & 90.59 (-0.72)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{3}{*}{\script{\citep{n29_liu2018rethinking}}}}  & \multicolumn{1}{c|}{VGG-19}                       & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{80\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.5}                  & 93.52 (+0.02)                     \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{PreResNet-110}                & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.04}                 & 95.06 (+0.02)                     \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{DenseNet-100}                 & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.24}                 & 95.21 (-0.03)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{2}{*}{\script{\citep{n33_dettmers2019sparse}}}} & \multicolumn{1}{c|}{VGG16-C}                      & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{93.51}                 & 93 (-0.51)                        \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{WRN-22-8}                     & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{95.74}                 & 95.07 (-0.67)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n40_choi2016towards}}}                     & \multicolumn{1}{c|}{ResNet-32}                    & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{77.8\%} & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.58}                 & 92.64 (+0.06)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n41_choi2020universal}}}                   & \multicolumn{1}{c|}{ResNet-32}                    & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{7.3\%}  & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.58}                 & 92.06 (-0.52)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n43_zhao2019variational}}}                   & \multicolumn{1}{c|}{ResNet-20}                        & \multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{16.47\%} & \multicolumn{1}{c|}{16.47\%\footnote{It has a sparse feature
			because it applies structured pruning on weight, which corresponds to
			channel pruning on feature.}} & \multicolumn{1}{c|}{92.01}                 & 91.66 (-0.35)                     \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n44_achterhold2018variational}}}           & \multicolumn{1}{c|}{DenseNet-76}                  & \multicolumn{1}{c|}{2}    & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{92.19}                 & 91.17 (-1.02)                     \\ \midrule
			\multicolumn{1}{c|}{\multirow{5}{*}{Ours}}                                    & \multicolumn{1}{c|}{\multirow{5}{*}{MobileNetV2}} & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{\multirow{5}{*}{92.6}} & \multicolumn{1}{c}{92.52 (-0.08)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{50\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.58 (-0.02)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{50\%} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.87 (-0.73)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{50\%}   & \multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{92.23 (-0.37)} \\
			\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   & \multicolumn{1}{c|}{--}     & \multicolumn{1}{c|}{50\%} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{91.65 (-0.95)} \\ \bottomrule
		\end{tabular}
	} 
	
	\caption[Caption for LOF]{Comparisons with previous pruning or quantization methods on
	CIFAR10. We argue our method stands strongly in performance against existing
	methods, but is far more versatile and robust\footnotemark.}
	\label{tb:cifar10_comp}
	% \vspace{-1em}
\end{table}

			

\footnotetext{Note that it is
	inherently difficult to compare different quantization and pruning methods
	because of diversity and difference between configurations. We continue this
	discussion in appendix~\ref{apn:benchmark}.}
					
					
					
					
					
\subsection{Object Detection}
\label{sec:exp_detection}
					
We conduct our objection detection experiment on Pascal VOC \citep{o_pascalvoc}
using Faster RCNN \citep{o_fasterrcnn} with a ImageNet \citep{o_imagenet}
pre-trained ResNet101 backbone. Since the original Faster RCNN trains on
images of different shapes each batch, it is impossible to obtain a fixed
unstructured pruning mask for convolution feature map as line 8 in
Alg.~\ref{alg:quantize}. Thus, for convolution feature, we apply structured
pruning. Note that we do not prune or quantize for the first 5
residual blocks because they are frozen originally and unfreezing
will collapse the training even for reference network. However, this
limitation can be easily overcome with group normalization or synchronized
batch normalization according to \citep{he2019rethinking}. Thus, we do not
regard this as our limitation.


Results of different configurations are shown in Table~\ref{tb:frcnn_main}. 
We compare with previous methods in Table~\ref{tb:frcnn_comp}. Contrary to existing methods like
\citep{detect_li2019fully}, which introduces major overhauls over the object
detection network training procedures, our method is less intrusive and works
without much modifications. Aligning with the original setting, we train with batch size equal to 1 and fix all
pre-trained batch normalization layers.
					
					
% \textbf{Performance.} It can be seen that we have the smallest performance
% loss among other methods, even when weight \& feature are quantized and weight
% are pruned 50\% (P-Q (W)). In the case of P-Q (F), we suffer a mAP drop of
% 1.47, but this is still smaller than that of
% \citep{n28_krishnamoorthi2018quantizing, detect_he2017channel}.
					 
% \textbf{Robustness.} Contrary to existing methods like
% \citep{detect_li2019fully}, which introduces major overhauls over the object
% detection network training procedures. Our method is less intrusive and works
% without much modifications. Aligning with the original setting, we train with batch size equal to 1 and fix all
% pre-trained batch normalization layers. Note that we do not prune or quantize for the first 5
% residual blocks because they are frozen originally and unfreezing
% will collapse the training even for reference network. However, this
% limitation can be easily discarded as long as group normalization or synchronized
% batch normalization according to \citep{he2019rethinking}. Thus, we do not
% regard this as our limitation.
					
% \textbf{Effect of Buffer Size.} From Table~\ref{tb:frcnn_main}, we can see that
% the mAP will drop 0.4 from P-Q (F) if we set $b_s$ to 1, which indicates that
% decimal bits $d$ and pruning mask $m$ can be more accurately computed from
% multiple batches especially when original batch size is small. 
					
% Furthermore, the training results are well reckoned in the summary 1.(a), 1.(c).
					
					
					  
\begin{table}[]
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{lrrrrrrrrr}
		\hline
		    & Reference & Q     & P  (W) & P  (F) & P-Q (F) & P-Q (F, BF=1) & P-Q (W) & Q-P (F) & Q-P (W) \\
		\hline
		MAP & 74.47     & 74.25 & 74.33  & 73.04  & 73      & 72.6          & 74.44   & 70.13   & 74.13   \\
		\hline
	\end{tabular}
	} \caption{Faster RCNN results with different prune \& quantization
	configurations on Pascal VOC 2007 test set. The
	non-commutativity persists in unstructured feature pruning.}
	\label{tb:frcnn_main}
\end{table}

	  
					  
\begin{table}[]
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{@{}cccccccc@{}}
		\toprule
		Method                           & Detection Framework          & W Bits & F Bits & W Sparsity & F Sparsity & Reference mAP          & mAP           \\ \midrule
		\script{\citep{n27_yang2019quantization}} & YOLO-v2                      & 8      & 8      & --         & --         & 72.64                  & 72.5 (-0.14)  \\ \midrule
		\script{\citep{n28_krishnamoorthi2018quantizing}} & SSD
		& 7      & 8      & --         & --         & 77.8                   &
		76.1 (-1.7)   \\ \midrule
		\script{\citep{detect_he2017channel}}  & Faster RCNN & -- & -- & --  & 50\% & 68.7
		& 66.9 (-1.8) \\ \midrule
		\script{\citep{detect_wei2018quantization}}  & Faster RCNN & 8 & 8 & --  & -- &
		44.6	  & 47.0 (+2.4) \\ \midrule
		\script{\citep{detect_yin2016quantization}}  & R-FCN & 6 & -- & --  & -- & 78.94
		& 78.24 (-0.7) \\ \midrule
		\multirow{3}{*}{Ours}            & \multirow{3}{*}{Faster RCNN} & 8      & 8      & --         & --         & \multirow{3}{*}{74.47} & 74.25 (-0.22) \\
		                                 &                              & 8      & 8      & 50\%       & --         &                        & 74.44 (-0.03) \\
		                                 &                              & 8      & 8      & --         & 50\%       &                        & 73 (-1.47)    \\ \bottomrule
	\end{tabular}
	} \caption{Comparisons with previous pruning or quantization methods on
	Pascal VOC 2007. We have the smallest performance loss among other methods.}
	\label{tb:frcnn_comp}
\end{table}

		  
					
\subsection{Super Resolution}
					
\label{sec:exp_sr}
					
We conduct our super resolution task on 91-image \citep{o_91image} (training set)
and Set5 \citep{o_set5} (validation set) with efficient sub-pixel convolution
network (ESPCN) \citep{espcn}, which is a 3-layer convolution network without
normalization layer. Results are summarized in Table~\ref{tb:sr_main}. Though every configuration
suffers a performance drop, our results still have better PSNR than the
original result reported in \citep{espcn} except for unstructured feature pruning cases.

% Note that we find the training is not stable enough.
% Therefore, for each configuration, we run five times and peak the best model, and
% the results are shown in Table~\ref{tb:sr_main}. 
					

					
% \textbf{Quantize helps Feature Pruning.} In this case, not only we find that it
% is more beneficial to quantize first and then prune, we also observe that
% feature pruning yields better performance with quantization. It indicates that
% the non-trivial relationship between quantization and feature pruning as we
% discussed in Sec.~\ref{sec:joint_pip}. This corresponds to summary 1.(c).
					
% \textbf{Gradient Peak.} In Fig.~\ref{fig:why_prune_then_quantize}, we show that
% feature pruning will incur gradient peaks. It is intuitive from hindsight since
% the network is trying to learn more by having large gradients when fractions of
% features suddenly become zero. This corresponds to summary 1.(b). 
					
\begin{table}[]
	\footnotesize
	\centering
	\begin{tabular}{rrrrrrrrrr}
		\hline
		Ref   & Q     & P  (W) & P  (F) & P-Q (W) & P-Q (F) & Q-P (W) & Q-P (F) \\
																	
		\hline
		32.86 & 32.69 & 32.77  & 31.52  & 32.57   & 31.7    & 32.59   & 32.12   \\
		\hline
	\end{tabular}
	\caption{PSNR (peek signal-to-noise ratio) with different prune \&
	quantization configurations on Set5. 
	In this experiment, we find the prune-then-quantize pattern is reversed and
	non-commutativity still holds. Moreover, quantization can even help unstructured feature
	pruning.}
	\label{tb:sr_main}
\end{table}
					
					
					
					
\begin{figure}[]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_feat.pdf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_grad.pdf}
		}
	\end{minipage}
																																						
	\caption{Take the super resolution task as an example, we visualize the
	gradient peak effect during unstructured feature pruning. This phenomenon is
	natural by hindsight and we consider it is generalizable to more scenarios.
	Gradients are sampled from feature.}
	\label{fig:why_prune_then_quantize}
\end{figure}
					
					
					
					
					
					
					
					
\subsection{Image to Image Translation and Generative Adversarial Network}
					
We conduct our image to image translation task on facades dataset with Pix2Pix
network \citep{pix2pix}, and our GAN task on horse2zebra dataset with CycleGAN
\citep{o_cyclegan}. Both of them applies an encoder-decoder structured network,
while the Pix2Pix uses UNet \citep{unet} and CycleGAN uses a variant of ResNet
with deconvolution layers. In Fig.~\ref{fig:pix2pix_demo} and
\ref{fig:cyclegan_demo}, we demonstrate some generated samples, and we provide
more samples in appendix~\ref{apn:more_demos}.
					
From Fig.~\ref{fig:pix2pix_demo}, it is hard to
distinguish the quality difference between the reference and quantized only
network, despite some color difference. If we add weight pruning, we can observe
some details get blurry. However, if we prune feature, though the overall
structure remains, the color becomes unnatural and some major distortions could
be spotted. From Fig.~\ref{fig:cyclegan_demo}, we can find that weight pruned
network transfers the texture correct but the color transfer seems unfinished,
while the feature pruned network looks like the opposite, which may represent a
division of functions within the network. 
					
\textbf{Feature Distribution and Information Granularity.} From
Fig.~\ref{fig:feat_histogram} and \ref{fig:cyclegan_demo} about CycleGAN, we are
amazed to discover that its feature distribution has a much longer tail, and its
generative quality is very sensitive to minor changes in feature, which
corresponds to to summary 2.
					
\begin{figure}[]
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.26}{
			\includegraphics{plots/pictures/pix2pix/main33/24.pdf}
		}
		\caption{Examples of generated images from Pix2Pix networks with different
		configurations. }
		\label{fig:pix2pix_demo}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.26}{
			\inputpgf{plots/pictures/cyclegan/main}{3.pgf}
		}
		\caption{Examples of generated images from CycleGAN networks with different
			configurations. 
			It is clear to see the saturated quantization works as an important factor,
		and more than 8 bits are required for this generative task.}
		\label{fig:cyclegan_demo}
	\end{minipage} 
\end{figure}
					
					
					
					
					
\begin{figure}[]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/feat_histogram_analysis/sr.pdf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/feat_histogram_analysis/cycle.pdf}
		}
	\end{minipage}
	\caption{Feature histogram comparison between the network of super
		resolution and CycleGAN. The features of
		CycleGAN are much more long-tailed, and our saturated quantization can
	handle well. }
	% 	Note that it is also natural to consider logarithmic
	% 	quantization for long-tailed distribution \citep{o_hubara2017quantized},
	% but it may result in additional difficulty for inference acceleration.
	\label{fig:feat_histogram}
\end{figure}
					
					
					
					
\section{Conclusion}
					
In this paper, we design a joint quantization and pruning methods, uncover
unstructured feature pruning as an important scenario for model compression
research and release our method as a software package. Moreover, we conduct
thorough experiments on a wide range of tasks and discover many interesting
findings.
					
Admittedly, this work bears its own limitations. We still could not fully
explain the complex inter-dependency between feature pruning and quantization,
and feature distribution of generative adversarial networks. Feature pruning
still suffers from non-negligible performance drop. However, we believe these
limitations could be regarded as future possibilities. It will be interesting to
see what could be built upon our findings.
					

==> include.backup0926/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[strings]{underscore}
% \usepackage{url}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{bbold}
\usepackage{graphicx}
\usepackage{fancybox}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage[noend,algoruled,linesnumbered, rightnl]{algorithm2e}
\usepackage{seqsplit}
\usepackage{multirow}
\usepackage{float}
\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{array}
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{multicol}
\usepackage{caption}
\usepackage{minted}
\usepackage{subcaption}
% \usepackage{algcompatible}
% \algnewcommand{\lst}{\texttt{lst}}
% \algnewcommand{\slst}{\texttt{slst}}
% \algnewcommand{\SEND}{\textbf{send}}

% \newsavebox{\algleft}
% \newsavebox{\algright}

\newtheorem{theorem}{Theorem}

\renewcommand{\url}[1]{\texttt{\seqsplit{#1}}}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rflo, rightnl}
\newcommand\tocite[1]{\textcolor{blue}{[#1]}}
\newcommand{\comment}[1]{}
\long\def\/*#1*/{}

\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


\newcommand{\python}[1]{
\inputminted[
frame=single,framesep=10pt,
bgcolor=lightergray,
fontsize=\footnotesize,
]{python}{#1}
}
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\SetKwInput{KwInput}{Input} % just a guess
\SetKwInput{KwOutput}{Output} % just a guess
\definecolor{lightergray}{RGB}{242, 242, 242}

\newcommand{\bsquare}{{\scriptsize $\blacksquare$}}
\newcommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\let\includegraphicsWithoutPath\includegraphics
\renewcommand{\includegraphics}[2][]{\includegraphicsWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}

\newcommand{\q}[1]{``#1''}

\newcommand{\ourlib}{\href{https://github.com/anonymous368/qsparse}{https://github.com/anonymous368/qsparse}}

\newcommand{\ourexamples}{\href{https://github.com/anonymous368/qsparse/tree/main/examples}{https://github.com/anonymous368/qsparse-examples}}

\newcolumntype{T}{>{\tiny}c}
\newcolumntype{S}{>{\scriptsize}c}

\newcommand{\script}[1]{{\scriptsize #1}}



==> include.backup1001/author.tex <==
\title{QSparse: Training Deep Neural Networks with Joint Quantization and Pruning of Features and Weights}

\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@eng.ucsd.edu}
	\And
	Ian Colbert\\
	UC San Diego\\
	\texttt{icolbert@eng.ucsd.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@eng.ucsd.edu} \\
	\And
	Srinjoy Das\\
	West Virginia University\\
	\texttt{srinjoy.das@mail.wvu.edu} 
}

\hypersetup{
pdftitle={QSparse: Training Deep Neural Networks with Joint Quantization and Pruning of Features and Weights},
pdfsubject={deep learning},
pdfauthor={Xinyu Zhang},
pdfkeywords={Quantization, Neural Networks, Pruning, Feature Pruning, Software Tool, Python, Pytorch, 
Model Compression, Object Detection, Super Resolution, Classification, Image to Image
Translation, Generative Adversarial Network, CycleGAN},
}

==> include.backup1001/body.tex <==
% QSparse: Training Deep Neural Networks with Joint Quantization and Pruning of
% Features and Weights

\begin{abstract}
				
	Quantization and pruning are widely used to reduce the inference costs of
	deep neural networks, but are typically treated as independent problems. In
	this work, we empirically evaluate this independence assumption across a
	wide range of computer vision tasks and observe interdependence and
	non-commutativity when applied to both features and weights. Informed by
	these observed dependencies, we propose a novel method to jointly train deep
	neural networks using both uniform quantization and unstructured pruning on
	both the features and weights. We demonstrate that our method delivers an
	increased performance per memory footprint over existing state-of-the-art
	solutions.
				
\end{abstract}
	
	
	
\section{Introduction}
\label{sec:intro}


Deep neural networks (DNN) have been widely deployed in various applications. 
To increase inference efficiency of DNN, quantization and pruning are important
techniques which have been studied extensively. 
Quantization \citep{n16_wu2020integer} reduces the bit-width required for weight and feature, which
enables us to accelerate DNN with fixed-point arithmetics and smaller memory footprint.
Pruning \citep{n35_hoefler2021sparsity} removes redundant parameters from weight, which decreases the overall
computational and memory requirements.


\textbf{Unstructured Feature Pruning.} Although there are many studies on
unstructured and structured weight pruning, to the best of our knowledge, no
attempt has been made to apply unstructured pruning on the feature map. However,
we argue that feature pruning is more beneficial than weight pruning from the
perspective of inference efficiency. Taking convolution as an example, skipping
a single output feature value can save an entire dot product
\citep{convarith_dumoulin2016guide}, while arbitrary weight sparsity cannot be
efficiently implemented on contemporary GPUs \citep{n13_gray2017gpu}. Moreover,
due to the prevalence of rectified activation functions \citep{xu2015empirical},
DNN feature are inherently sparse \citep{glorot2011deep}. Except that the sparse
pattern is not pre-determined but depends on each input, thus making it
difficult to utilize.


\textbf{Relation between Quantization and Pruning.} Pruning and quantization are
often considered to be able to solve independently \citep{n21_liang2021pruning}.
Though there have been some recent research to study both quantization and
pruning in a unified scope, they generally assume a Prune-then-Quantize paradigm
without enough investigation on other choices \citep{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint}.  
However, after taking feature pruning into consideration, we find that the
temporal order of quantization and pruning becomes a critical factor. These
operations become non-commutative, and exchanging the order of pruning and
quantization can lead to catastrophic performance degradation. Moreover, feature
pruning can only lead to proper convergence when used in conjunction with
quantization in certain important scenarios.


\textbf{Quantization and Pruning Method.} Most existing work focus on image
classification, and some work have covered object detection
\citep{detect_li2019fully}. However, this study has not yet but should be
generalized to a broader range of computer vision (CV) tasks. For example,
pruning and quantization research on generative tasks like generative
adversarial network (GAN) is still limited to weight quantization
\citep{n23_wang2019qgan} and sparse regularization \citep{n34_zhou2020sparse}.



\textbf{Contributions.}

	
\begin{enumerate}
	\item To the best of our knowledge, this is the first work that studies
	      unstructured feature pruning extensively. Contrary to the independence
	      assumption, we empirically show interdependence and non-commutativity
	      between pruning and quantization when applied to both features and weights.
	      	      	      
	\item We propose a novel method to jointly train deep neural networks using
	      both uniform quantization and unstructured pruning on both the features and
	      weights. We show that our method delivers the best performance per memory
	      footprint over existing state-of-the-art solutions, and supports a wide
	      range of computer vision applications over image classification, object
	      detection, super resolution, Pix2Pix \citep{pix2pix} and CycleGAN
	      \citep{o_cyclegan}.
	      	      	      	      	      	      	      	      	      																																																																																																																																																																																																																															  
	\item We release our method as a pytorch-based python package \ourlib. With a
	      completely innovative design, our library is compatible with any pytorch
	      modules.
\end{enumerate}





\section{Unstructured Feature Pruning}

Let $L \in \mathbb{N}^+$ denote the number of layers in a DNN, $x_i,
i\in\{1,...,L\}$ be the output feature map of layer $i$, $x_0$ be the DNN input, $T_i(x)$ be
the computation function of layer $i$, such as convolution or matrix-vector
multiplication, $\sigma$ be the activation function, then a DNN can be written
as a function $F$ in Eq.~\ref{eq:dnn}:

\begin{equation}
	x_L \mapsto F(x) := T_L(\sigma(T_{L-1}(... \sigma(T_1(x_0)) ... )))
	\label{eq:dnn}
\end{equation}

We define \textit{unstructured feature pruning} as an element-wise multiplication between
feature map and a binary mask. Specifically, let $\mathring{x}_i$ be the pruned
output feature of layer $i$, and $\mathring{m}_i$ be the binary mask for layer
$i$ with the same shape as $x_i$, then we can write the pruning operation for
$x_i$ as $P_i$ in Eq.~\ref{eq:fp}:

\begin{equation}
	\mathring{x}_i \mapsto P_i(x) := x \, \mathring{m}_i
	\label{eq:fp}
\end{equation}

Therefore, based on $P_i$ in Eq.~\ref{eq:fp}, we can write the function of a
feature-pruned DNN as $\mathring{F}$ in Eq.~\ref{eq:fpdnn}:

\begin{equation}
	\begin{split}
		\mathring{F}(x) & := T_L(\sigma(\mathring{T}_{L-1}(... \mathring{T}_2(\sigma(T_1(x_0))) ... ))) \\
		\text{where } \mathring{T}_i(x) & = P_i(T_i(x))
	\end{split}
	\label{eq:fpdnn}
\end{equation}

We prune the output feature maps of all layers from $2$ to $L-1$ and skip the
first and last layer. In this paper, we assume that $\mathring{m}_i$ belongs to network parameters and
doesn't change with $x_0$. Therefore, we could skip the computation of values in
$x_i, i \in \{2,...,L-1\}$ whose corresponding mask is 0 in $\mathring{m}_i$ during inference.


\section{Method}
\label{sec:method}

We design our method with two components, quantization operator and pruning
operator, both of which can work independently on either weight (W) or feature (F).
Based on these two operators, we outline a jointly pruned and quantized layer on
both weight and feature as
shown in Fig.~\ref{fig:pipeline}, where pruning is applied before quantization
structurally as \citep{n17_yu2020joint} has explained the benefit that pruning
can help to reduce quantization error because 0 can always be perfectly
quantized. 


\begin{figure}[]
	\centering
	\includegraphics[width=0.7\linewidth]{plots/conv.pdf}
	\caption{An example of applying joint pruning and quantization of both
		weight and feature on a
	convolution layer.}
	\label{fig:pipeline}
\end{figure}


Because of the temporal interdependence as shown in Sec.~\ref{sec:relation}, we
enable these two operators to cooperate in the temporal dimension by controlling
$t_q$ in Alg.~\ref{alg:quantize} and $t_0 + n\Delta t$ in Alg.~\ref{alg:prune}
without explicitly setting a pre-defined order.



\subsection{Quantization Operator}

Our quantization operator is an improved version from
\citep{o_hubara2017quantized}, by which they both leverage "straight-through
estimator" for gradient calculation and follow a inference-friendly uniform 
quantization scheme \citep{n25_jacob2018quantization}. Giving input $x_t$ to
denote either weight or feature at step $t$, $N$ be the total number of
bits, $d$ be the number of decimal bits\footnote{Bits used to represent
	fractions}, the quantized $x_t$ can be represented by $\hat{x}_t$:
					
					
\begin{equation}
	\begin{split}
		\hat{x}_t & = \text{clip}(\floor{x_t * 2^{d}}, -2^N, 2^N-1) / 2^d \\
		\frac{\partial Loss}{\partial x_t} & = \text{clip}(\frac{\partial Loss}{\partial \hat{x}_t}, -2^{N-d}, 2^{N-d} - 1)
	\end{split}
	\label{eq:quantize}
\end{equation}
					
					
However, we make two simple yet effective enhancements on top of existing methods, as
explained below and Alg.~\ref{alg:quantize}. 


					
\begin{enumerate}
	\item \textbf{Delayed Quantization.} Instead of using floating point auxiliary weights for simulated
	      quantization \citep{n25_jacob2018quantization} or finding clever weight
	      initialization \citep{o_init_q}, we start by training the original float network, then calculate the optimal decimal
	      bits by minimizing the quantization error after a given number of
	      steps $t_q$. By thorough experiments in Sec.~\ref{sec:exp}, we
	      show that our method achieves superior performance while 
	      accommodating initialization and training dynamics of various applications.
	      	      	      	      		      		      		      		      																																																																																																																																																																																																																															  
	\item \textbf{Saturated Quantization.} When calculating the optimal decimal bits, instead of using the
	      standard mean square quantization error $\arg \min_{d} |\hat{x}_t - x_t|^2$,
	      we saturate $x_t$ to protect the quantization from outliers:
	      	      	      	      		      		      		      		      																																																																																																																																																																																																																															  
	      \begin{equation}
	      	\begin{split}
	      		d^* & = \arg \min_{d} |\hat{x}_t - \text{saturate}(x_t)|^2 \\
	      		\text{saturate}(x) & = \text{clip}(x, \text{quantile}(x, s_l), \text{quantile}(x, s_u)) \\
	      		\text{quantile}(x, a) & =  a\text{-th quantile of } x \\
	      		s_l, s_u & \in [0, 1], s_l < s_u
	      	\end{split}
	      	\label{eq:qmse}
	      \end{equation}
	      	      	      	      		      		      		      		      																																																																																																																																																																																																																															  
	      We show that the saturated quantization is critical for feature
	      quantization in applications like CycleGAN from Fig.~\ref{fig:saturated_quantize}.  % fig:cyclegan_demo
\end{enumerate}

\begin{figure}[]
	\begin{minipage}[t]{0.39\linewidth}
		\scalebox{0.29}{
			\includegraphics{plots/pictures/feat_histogram_analysis/together.pdf}
		}
	\end{minipage}%
	% \hfill%
	\begin{minipage}[t]{0.58\linewidth}
		\scalebox{0.325}{
			\includegraphics{plots/pictures/cyclegan/saturation/3.pdf}
		}
								
	\end{minipage} 
	\caption{Feature distribution and generated images from CycleGAN networks.
		We can see that the feature distribution of CycleGAN are much more
		long-tailed, while our saturated quantization can handle well. We
		quantize features of CycleGAN with 12 bit.}
	\label{fig:saturated_quantize}
\end{figure}
			

\subsection{Pruning Operator}

Our pruning operator is an improved version from \citep{n45_zhu2017prune}.
Specifically, it is an automated gradual pruning algorithm where the
sparsity is increased during training for $n$ repetitions till the final
sparsity $s_f$. Let $\Delta t$ be the interval between each pruning step,
$t_0$ be the start step of the pruning procedure, the sparsity at time $t$
is denoted by $s_t$ in Eq.~\ref{eq:sparsity}.
					
\begin{equation}
	s_{t}=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta t}\Bigr\rfloor\right)^{\gamma} \right) 
	\label{eq:sparsity}
\end{equation}
					
At each pruning step when $t = t_0 + i \Delta t, i\in [n]$, a mask $m_t$ is
calculated by zeroing out the smallest magnitude input until the $s_t$ is
reached. $\gamma$ is usually set to 3 based on empirical analysis. This mask
will be kept the same for both training and inference until the next pruning
step if exists. 
					
\begin{wraptable}[5]{l}{17em}
	\footnotesize
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Faster RCNN}                                 & \textbf{mAP} \\ \hline
		(1) Float + Dense                                    & 74.47        \\ \hline
		\begin{tabular}[c]{@{}l@{}}(2) Quantize + 50\% Prune  \\ \hspace{1em} on W, F ($b_f$ = 32)\end{tabular} & 73 (-1.47)   \\ \hline
		(3) Like (2), but $b_f$ = 1                          & 72.6 (-1.87) \\ \hline
	\end{tabular}
	\caption{Results of quantized and pruned Faster RCNN on Pascal VOC 2007 test set with different buffer size $b_f$.}
	\label{tb:frcnn_bf}
\end{wraptable}	


% for feature pruning
The modification we make is instead of only depending on magnitude of the
current input, during feature pruning, we maintain an input buffer so we construct the mask from the
magnitude of a history of features. We see that the input buffer is important for
unstructured feature pruning in Table~\ref{tb:frcnn_bf}. 


					
					
						
\begin{figure}[]
	\begin{minipage}[t]{0.48\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\SetNlSkip{0em}
			\KwInput{number of bits $N$, quantize step $t_q$ \\ \hspace{2em} saturation range $s_l,
			s_u$}     % , buffer size $b_f$
			\KwOutput{decimal bits $d$}
			% $B \gets $ empty queue with size $b_f$\\
			$d \gets 0$ \\
			\For{$t \gets 1$ to $T$}{
				\eIf{$t < t_q$}{
					$o_t \gets x_t$	
					}{
					\If{$t\equiv t_q$}{$d \gets $ calculate from $x_t, s_l, s_u$ \\ 
						\hspace{2em} with Eq.~\ref{eq:qmse}}
					$o_t \gets \text{clip}(\floor{x_t * 2^{d}},$ \\
					\hspace{4em} $-2^N, 2^N-1) / 2^d$
				}
			}
			\caption{Quantize Operator}
			\label{alg:quantize}
		\end{algorithm} 
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.48\textwidth}
		\begin{algorithm}[H]
			\SetAlgoLined
			\KwInput{sparsity $s_f$, start step $t_0$, interval $\Delta t$ \\
				\hspace{3em} repetition $n$, buffer size $b_f$}     
			\KwOutput{mask $m_T$}
																																																																																																																						
			$B \gets $ empty queue with size $b_f$\\
			$s_0 \gets 0$ and $m_0 \gets \mathbb{1}$ \\
			\For{$t \gets 1$ to $T$}{
				append $x_t$ to B \\
				$s_{t}=s_{f} \Big(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta
					t}\Bigr\rfloor\right)^{3} \Big)$ \\
				\eIf{$s_{t-1} \neq s_t$}{
					$m_t \gets $ calculate mask from $B$ and $s_t$
					}{
					$m_t \gets m_{t-1}$
				} 
				$o_t \gets x_t * m_t$
			}
			\caption{Pruning Operator}
			\label{alg:prune}
		\end{algorithm} 
	\end{minipage}
\end{figure}	
% \end{multicols}
					
				
					 
Giving input $x_t$ to denote either weight or feature at step $t$, $T$ as
the total number of steps, $o_t$ to denote the operator output, the pruning
operator mechanism is demonstrated in Alg.~\ref{alg:prune}. The mask
calculation in line 8 will find the positions with smallest magnitude
averaged over a buffer of history inputs.

\section{Relation between Quantization and Pruning}
\label{sec:relation}


Based on Sec.~\ref{sec:method}, we could jointly schedule two operators by
controlling the relationship between $t_0 + n\Delta t$ in Alg.~\ref{alg:prune}
and $t_q$ in Alg.~\ref{alg:quantize} for both weight and feature. While previous
methods generally assume a Prune-then-Quantize paradigm ($t_0 + n\Delta t <
t_q$), we find this argument is not sufficient to depict the relationship
between pruning and quantization when applied to both weight and feature.


\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|l|}
				\hline
				\textbf{(a) MobileNetV2}    & \textbf{Top-1 Acc} \\ \hline
				Float + Dense           & 92.6               \\ \hline
				Prune-Quantize (W, F)   & 91.44 (-1.16)      \\ \hline
				Quantize-Prune (W, F)   & 86.84 (-5.76)      \\ \hline
				Prune(W)-Quantize(W, F) & 92.23 (-0.37)      \\ \hline
				Quantize(W, F)-Prune(W) & 85.94 (-6.66)      \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|l|}
				\hline
				\textbf{(b) Faster RCNN}    & \textbf{mAP}  \\ \hline
				Float + Dense           & 74.47         \\ \hline
				Prune-Quantize (W, F)   & 73 (-1.47)    \\ \hline
				Quantize-Prune (W, F)   & 70.13 (-4.34) \\ \hline
				Prune(W)-Quantize(W, F) & 74.44 (-0.03) \\ \hline
				Quantize(W, F)-Prune(W) & 74.13 (-0.34) \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|l|}
				\hline
				\textbf{(c) ESPCN}          & \textbf{PSNR} \\ \hline
				Float + Dense           & 32.84         \\ \hline
				Prune-Quantize (W, F)   & 31.03 (-1.81) \\ \hline
				Quantize-Prune (W, F)   & 31.66 (-1.18) \\ \hline
				Prune(W)-Quantize(W, F) & 32.51 (-0.33) \\ \hline
				Quantize(W, F)-Prune(W) & 32.54 (-0.30) \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize Comparison between Prune-then-Quantize (P-Q) with
	Quantize-then-Prune (Q-P) in
	(a) image classification with MobileNetV2 on CIFAR10, (b) objection detection with
	Faster RCNN on Pascal VOC, and (c) super resolution with ESPCN \citep{espcn} on
	Set5 (from left to right). Note that \q{Prune-Quantize (W, F)} represents
	8bit quantization and 50\% sparsity pruning on both weight and feature in
	Prune-then-Quantize order, \q{Quantize(W, F)-Prune(W)} means 8bit
	quantization on weight and feature, and 50\% sparsity pruning on weight only
	in Quantize-then-Prune order, the same rule applies for others.}
	\label{tb:non-comu}
\end{table}



\textbf{Non-commutativity.} In Table.~\ref{tb:non-comu}, we can see that the P-Q
pattern generally holds for weight-only pruning, while the difference between
P-Q and Q-P is minimal, which means these two operations are actually commutative in
these scenarios. However, we observe a sharp difference between P-Q and Q-P when
including feature pruning. In (a) and (b), P-Q outperforms Q-P by a large
margin, while (c) shows this relationship in the opposite direction. This is to
say, pruning and quantization become non-commutative and exchanging the correct
order of pruning and quantization can lead to catastrophic performance
degradation. 

\begin{wraptable}[10]{r}{17em}
	\footnotesize
	\begin{tabular}{|l|l|}
		\hline
		\textbf{ESPCN}            & \textbf{PSNR} \\ \hline
		Float + Dense             & 32.84         \\ \hline
		Prune (F) Only            & 31.36 (-1.48) \\ \hline
		Quantize (W, F)            & 32.68 (-0.16) \\ \hline
		Quantize (W, F)-Prune (F) & 32.03 (-0.81) \\ \hline
	\end{tabular}
	\caption{Comparison between unstructured feature pruning only and pruning
	with quantization in super resolution task.}
	\label{tb:interdependence}
\end{wraptable}

\textbf{Interdependence.} In Table.~\ref{tb:interdependence}, we even find that
feature pruning even provides better performance over a quantized network
instead of a floating-point network for our super resolution experiment. We
didn't observe this phenomenon in other experiments.



\textbf{Gradient Spike Effect.} Furthermore, we provide a gradient perspective
to explain our observations. In Fig.~\ref{fig:gspike}, we find that pruning will
incur spikes on gradient of activations when operating on feature because loss
will be more concentrated on the remaining values. We suppose this could even be
exacerbated through back-propagation. Moreover, the gradient peak could
correlate with two additional dynamics: (1) the gradient clamping from
straight-through gradient estimator in Eq.~\ref{eq:quantize}. (2) gradient of
the origin model. Networks could converge differently based on the tension
among these dynamics.



\begin{figure}[]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_feat.pdf}
		}
	\end{minipage}%
	\begin{minipage}{.5\textwidth}
		\centering
		\scalebox{0.5}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_grad.pdf}
		}
	\end{minipage}
																																									
	\caption{Visualization of
	gradient peak effect during unstructured feature pruning.}
	\label{fig:gspike}
\end{figure}
					
					




\section{Software Interface}


We release our method in a pytorch-based software package. In
Listing~\ref{code:interface}, we demonstrate how simple and flexible it can make
pruned and quantized training to be. Unlike existing libraries
\citep{t_xilinx,QatTorch} that only provides a limited set of quantized or
pruned layers isolated from other modules, our library directly transforms the
weight attribute of the input layer into a quantized or pruned version during
runtime. This is to say, our library is layer-agnostic and can work with any
pytorch modules, as long as their parameters can be accessed from the weight
attribute. More information can be found at \ourlib.


\section{Experiments}
\label{sec:exp}
% - cite appendix
% - 12bits results + pix2pix
% - explain some experiment settings
% - state convention (8bit, 50%)

To evaluate our method, we conduct experiments on five tasks: image
classification, object detection, super resolution, image to image translation,
and generative adversarial network. For each task, if not specifically stated,
we apply 8-bit quantization on both feature and weight of every layer,
unstructured pruning with sparsity of 50\% on feature and weight except the
first \& last layer. Here we focus on two configurations: (1) pruning and
quantization on both weight \& feature, (2) pruning on weight and quantization
on feature and weight. We provide results of more configurations in
Appendix~\ref{apn:more_exp}.


We implement each task by applying minimal code changes with our library on top
of existing popular open-source implementations. We maintain hyper-parameters
identical to the original settings except for training epochs and when to apply
quantization \& pruning. More details about experiment setups are available in
appendix~\ref{apn:detailed_exp}. We release all experiment source code as
examples for our library.


\textbf{Image Classification.}  We conduct our image classification task on
CIFAR10 \citep{o_cifar10} with MobileNetV2 \citep{mobilenetv2}. We compare with
previous methods in Table~\ref{tb:cifar10_comp} in terms of memory footprint and
\textit{performance density}, a metric we introduce to fairly compare various
methods under a unified scope. We calculate the memory footprint of a model by
summing the size of its parameters and feature maps. We define the
\textit{performance density} of a model by dividing its accuracy by memory
footprint. 

% With joint pruning and quantization on both weight and feature, we
% achieve the best memory footprint and performance density
					

\begin{table}[]
	\centering
	\vspace{-1em}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccccccccc}
			\toprule
			Method
			& Network                                           & W Bits
			& F Bits                   & W Sparsity                  & F
			Sparsity                & Ref Acc                               &
			\multicolumn{1}{c}{Accuracy}  & \multicolumn{1}{c}{\scriptsize \begin{tabular}[c]{c}Memory \\ Footprint (Mb) \end{tabular}} &
			\multicolumn{1}{c}{\scriptsize \begin{tabular}[c]{c}Performance \\ Density (Acc/Mb) \end{tabular}}   \\
			\midrule
			\multicolumn{1}{c|}{\script{\citep{n2_yang2020automatic}}}
			& \multicolumn{1}{c|}{ResNet-20}                    &
			\multicolumn{1}{c|}{1.9}  & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{91.29}                 & 91.15 (-0.14)  & 88.41 & 1.03  \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n3_xiao2019autoprune}}}
			& \multicolumn{1}{c|}{VGG-16}                       &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{79\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.4}                  & 91.5 (-1.9)        &
			134.36 & 0.68		\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n4_van2020bayesian}} }
			& \multicolumn{1}{c|}{VGG-7}                        &
			\multicolumn{1}{c|}{4.75} & \multicolumn{1}{c|}{5.4} &
			\multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.05}                 & 93.23 (+0.18)
			&  47.12 & 1.98		\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n24_paupamah2020quantisation}}}
			& \multicolumn{1}{c|}{MobileNet}                    &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{91.31}                 & 90.59 (-0.72)        &
			38.91 & 2.33		\\ \midrule
			\multicolumn{1}{c|}{\multirow{3}{*}{\script{\citep{n29_liu2018rethinking}}}}
			& \multicolumn{1}{c|}{VGG-19}                       &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{80\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.5}                  & 93.52 (+0.02)       &
			167.06 & 0.56          \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{PreResNet-110}                &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.04}                 & 95.06 (+0.02) &
			1571.74 & 0.06             \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{DenseNet-100}                 &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.24}                 & 95.21 (-0.03)  &  453.84 & 0.21                \\ \midrule
			\multicolumn{1}{c|}{\multirow{2}{*}{\script{\citep{n33_dettmers2019sparse}}}}
			& \multicolumn{1}{c|}{VGG16-C}                      &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.51}                 & 93 (-0.51)   &  58.96 & 1.58                  \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{WRN-22-8}                     &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.74}                 & 95.07 (-0.67)     &
			258.15 & 0.37		\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n40_choi2016towards}}}
			& \multicolumn{1}{c|}{ResNet-32}                    &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{77.8\%} & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.58}                 & 92.64 (+0.06)    &
			168.87 & 0.55			\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n41_choi2020universal}}}
			& \multicolumn{1}{c|}{ResNet-32}                    &
			\multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{87.5\%}  & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.58}                 & 92.57 (-0.01)    &
			152.35 & 0.61			\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n43_zhao2019variational}}} & \multicolumn{1}{c|}{DenseNet-40} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{59.67\%} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{94.11} 
			& 93.16 (-0.95)    & 118.10 & 0.79               \\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n44_achterhold2018variational}}}
			& \multicolumn{1}{c|}{DenseNet-76}                  &
			\multicolumn{1}{c|}{2}    & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.19}                 & 91.17 (-1.02)  &  283.21 & 0.32                 \\ \midrule
			\multicolumn{1}{c|}{\multirow{2}{*}{Ours}}
			& \multicolumn{1}{c|}{\multirow{2}{*}{MobileNetV2}} &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{\multirow{2}{*}{92.6}} &
			\multicolumn{1}{c}{92.23 (-0.37)} & 64.39 & 1.43 \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{}                             &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{50\%} &
			\multicolumn{1}{c|}{}                      &
			\multicolumn{1}{c}{91.44 (-1.16)} &  \textbf{36.79} & \textbf{2.49} \\ \bottomrule
		\end{tabular}
	} 
					
	\caption{Comparisons with previous pruning or quantization methods on
	CIFAR10. Our method provides the smallest memory footprint and best
	performance density and is far more versatile.}
	\label{tb:cifar10_comp}
\end{table}

\textbf{Object Detection.} 
We conduct our objection detection experiment on Pascal VOC \citep{o_pascalvoc}
using Faster RCNN \citep{o_fasterrcnn} with a ImageNet \citep{o_imagenet}
pre-trained ResNet101 backbone. Results can be found in Table~\ref{tb:non-comu}.
Since the original Faster RCNN trains on images of different shapes each batch,
it is impossible to obtain a fixed unstructured pruning mask for convolution
feature map as line 8 in Alg.~\ref{alg:quantize}. Thus, we apply channel-wise
pruning on convolution feature. Note that we do not prune or quantize for the
first 5 residual blocks because they are frozen originally and unfreezing will
collapse the training even for float dense network. However, this limitation can
be easily overcome with group normalization or synchronized batch normalization
according to \citep{he2019rethinking}. Thus, we do not regard this as our
limitation. Contrary to existing methods like \citep{detect_li2019fully}, which
introduces major overhauls over the object detection network training
procedures, our method is less intrusive and works without much modifications.
Aligning with the original setting, we train with batch size equal to 1 and fix
all pre-trained batch normalization layers.


\begin{figure}[]
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.265}{
			\includegraphics{plots/pictures/pix2pix/both/24.pdf}
		}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.265}{
			\includegraphics{plots/pictures/cyclegan/both/3.pdf}
		}
								
	\end{minipage} 
	\caption{Examples of generated images from Pix2Pix (left) and CycleGAN
	(right) networks. We quantize the features of Pix2Pix with 8bit and features
	of CycleGAN with 12bit.}
	\label{fig:pix2pix_cyclegan}
\end{figure}

\textbf{Super Resolution.} 
We conduct our super resolution task on 91-image \citep{o_91image} (training
set) and Set5 \citep{o_set5} (validation set) with efficient sub-pixel
convolution network (ESPCN) \citep{espcn}, which is a 3-layer convolution
network without normalization layer. Results can be found in
Table~\ref{tb:non-comu} and \ref{tb:interdependence}. Though every configuration
suffers a performance drop, the result of Quantize(W,F)-Prune(W) almost has the
identical PSNR with the original result reported in \citep{espcn}.


\textbf{Pix2Pix and CycleGAN.} We conduct our image to image translation task on
facades dataset with Pix2Pix network \citep{pix2pix}, and our GAN task on
horse2zebra dataset with CycleGAN \citep{o_cyclegan}. Both of them applies an
encoder-decoder structured network, while the Pix2Pix uses UNet \citep{unet} and
CycleGAN uses a variant of ResNet with deconvolution layers. Some generated
samples are demonstrated in Fig.~\ref{fig:pix2pix_cyclegan}, and we provide more
samples in appendix~\ref{apn:more_demos}. For Pix2Pix, it is hard to distinguish
the quality difference between samples of (1) and (2). If we add feature
pruning, though the overall structure remains, the color becomes unnatural and
some major distortions could be spotted. For CycleGAN, we find the feature map
needs more than 8bit (we use 12bit) to deliver decent generative results.

					

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion and Future Work}

We only evaluate our method and findings on computer vision tasks with a limited set of
neural architectures and relatively smaller datasets. In future work, we intend
to try more network structures like transformer \citep{NIPS2017_3f5ee243} and 
larger datasets, e.g. ImageNet \citep{o_imagenet}, Coco
\citep{lin2014microsoft}, Cityscape \citep{Cordts2016Cityscapes}, and more tasks
such as natural language processing.

\textbf{Parameterized Feature Pruning.} In this work, we assume that the feature
binary mask $\mathring{m}_i$ in Eq.~\ref{eq:fp} belongs to network parameters
and does not depend on current input. However, we haven't explored the
possibility to enable sparsity pattern in $\mathring{m}_i$ to condition on
network input $x_0$. This may not be practical to weight pruning but it is
likely to work for feature pruning, according to \citep{yang2019condconv} which
designs parameterized convolutions with a similar idea. 

% regularized layer inter dependence
\textbf{Joint Feature Pruning on Multiple Layers.} We only learn pruning mask
independently for each feature map. However, contrary to network weights,
feature maps are more correlated with each other. A good example for the
inter-layer correlation is the receptive field for convolution network, which
grows larger as network depth increases but keeps its center position unchanged.
This could give us an insight that we shall jointly consider multiple layers to
reduce the overall costs on accuracy instead of relying on local optimum at each
layer.


\textbf{Understanding Feature Pruning Behavior.} In Sec.~\ref{sec:relation}, we
see that feature pruning brings about some interesting relationships between
quantization and pruning. Though we provide a gradient-based explanation, it is
not nearly enough. Moreover, from Sec.~\ref{sec:exp}, we can tell that feature
pruning always yields a much larger accuracy penalty than weight pruning and
quantization. In future work, we need to develop more theoretical results to
provide intuitions and understanding. 

% understanding feature pruning (is more difficult)
% pruning on generative model
%  - whether magnitude base pruning will still work for generative pruning?

\textbf{Inference Acceleration for Feature Pruned Networks.} In
Sec.~\ref{sec:intro}, we briefly argue the potential benefits of applying
unstructured pruning on feature over weight. By taking convolution as an
example, we can easily see that skipping a single output feature value can save
an entire dot product. However, we acknowledge that our argument is far from
enough for real-world applications. We are looking forward to work on
specialized hardware or software implementations that realize the advantages of
feature pruning.




\section{Related Work}

\label{sec:relate}
				
Due to space limit and the fact that both quantization and pruning are large areas of research
with broad practical impacts, we will only outline concepts and work closely related to our contributions
in this section. We provide an extended review in appendix~\ref{apn:related_work}.
				
					
\textbf{Quantization.} Quantization \citep{n16_wu2020integer} is the process
of quantifying floating numbers with integer equivalents and can be applied
on both weights and feature. Post-training quantization
\citep{n26_lee2018quantization} aims on converting a trained float network
to quantized version without adequate access to training data, which is
convenient but sometimes suffers from accuracy degradation.
Quantization-aware training \citep{o_hubara2017quantized} involves
quantization into the training process, which usually provides better
accuracy but requires more efforts. Most work are focused on classification
tasks, while there are some recent work \citep{detect_wei2018quantization,
detect_li2019fully} on quantization for objection detection networks.
\citep{n23_wang2019qgan} quantizes the weight of a GAN to low bit-width on
CIFAR10 and CelebA \citep{o_celebA}.
					
				
					
					
\textbf{Pruning.} Sparsity is a long-standing research problem in the neural
network domain \citep{n38_gale2019state, n35_hoefler2021sparsity}, and
pruning is an important technique to obtain sparse neural network by
removing unimportant connections. Finetuning-based methods prune gradually
during training \citep{n45_zhu2017prune}, and retraining-based methods
retrain networks with pruned structure \citep{n37_frankle2018lottery}. There
have been debates about which one is better \citep{n29_liu2018rethinking,
renda2020comparing}. Most of known pruning methods act on weight, and can be
categorized as structured \citep{o_liu2017learning} and unstructured pruning
\citep{o_han2015learning}, while the former one requires to removes a
channel of weight together and the latter one can remove weight arbitrarily.
Most work are focused on classification tasks, and
\citep{detect_he2017channel} proposes a layer-wise structured pruning method
for object detection. There are some work connects GAN with sparsity
\citep{n34_zhou2020sparse}, but their focus is to use sparse
regularization to improve generative quality instead of pruning.
				
				
					
\textbf{Joint Quantization and Pruning.} There are relatively few work that
jointly consider pruning and quantization. Most work assumes a
Prune-then-Quantize pipeline \citep{n8_han2015deep, n10_zhao2019focused,
n17_yu2020joint}. \citep{n21_liang2021pruning, n24_paupamah2020quantisation}
further claim that pruning and quantization can be studied independently. 

\textbf{Neural Architecture Search.} There are some recent research that applies
neural architecture search (NAS) to discover high-performing networks with
quantization and pruning \citep{wang2020apq}. \citep{wu2018mixed} employs NAS to find mixed
precision networks which assign different bit-width for each convolution kernel.
\citep{cai2019once} uses pruning as a NAS primitive and trains one large network
and prunes it to accommodate different hardware settings. We argue that our work
is complementary to this direction because a NAS pipeline could build upon
different quantization and pruning methods.



					
				
					
					
\textbf{Neural Network Compression Toolbox.} There are many open-source
model compression tools that provide pruning or quantization functionality.
However, as far as our best knowledge, none of them offer joint pruning \&
quantization. Moreover, many tools are designed to be heavily inflexible and
some even requires developers to write code in a domain-specific language
(DSL). We discuss this more details in appendix~\ref{apn:related_work}.

==> include.backup1001/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[strings]{underscore}
% \usepackage{url}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{bbold}
\usepackage{graphicx}

\usepackage{fancybox}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage[noend,algoruled,linesnumbered, rightnl]{algorithm2e}
\usepackage{seqsplit}
\usepackage{multirow}
\usepackage{float}
\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{array}
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{multicol}
\usepackage{caption}
\usepackage{minted}
\usepackage{subcaption}
\usepackage{accents}
% \usepackage{algcompatible}
% \algnewcommand{\lst}{\texttt{lst}}
% \algnewcommand{\slst}{\texttt{slst}}
% \algnewcommand{\SEND}{\textbf{send}}

% \newsavebox{\algleft}
% \newsavebox{\algright}

\newtheorem{theorem}{Theorem}

\renewcommand{\url}[1]{\texttt{\seqsplit{#1}}}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rflo, rightnl}
\newcommand\tocite[1]{\textcolor{blue}{[#1]}}
\newcommand{\comment}[1]{}
\long\def\/*#1*/{}

\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


\newcommand{\python}[1]{
\inputminted[
frame=single,framesep=10pt,
bgcolor=lightergray,
fontsize=\footnotesize,
]{python}{#1}
}
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\SetKwInput{KwInput}{Input} % just a guess
\SetKwInput{KwOutput}{Output} % just a guess
\definecolor{lightergray}{RGB}{242, 242, 242}

\newcommand{\bsquare}{{\scriptsize $\blacksquare$}}
\newcommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\let\includegraphicsWithoutPath\includegraphics
\renewcommand{\includegraphics}[2][]{\includegraphicsWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}

\newcommand{\q}[1]{``#1''}

\newcommand{\ourlib}{\href{https://github.com/anonymous368/qsparse}{https://github.com/anonymous368/qsparse}}

\newcommand{\ourexamples}{\href{https://github.com/anonymous368/qsparse/tree/main/examples}{https://github.com/anonymous368/qsparse-examples}}

\newcolumntype{T}{>{\tiny}c}
\newcolumntype{S}{>{\scriptsize}c}

\newcommand{\script}[1]{{\scriptsize #1}}



==> include.backup1002/author.tex <==
\title{QSparse: Training Deep Neural Networks with Joint Quantization and Pruning of Features and Weights}

\author{Xinyu Zhang\\
	UC San Diego\\
	\texttt{xiz368@eng.ucsd.edu}
	\And
	Ian Colbert\\
	UC San Diego\\
	\texttt{icolbert@eng.ucsd.edu} \\
	\And
	Ken Kreutz-Delgado\\
	UC San Diego\\
	\texttt{kreutz@eng.ucsd.edu} \\
	\And
	Srinjoy Das\\
	West Virginia University\\
	\texttt{srinjoy.das@mail.wvu.edu} 
}

\hypersetup{
pdftitle={QSparse: Training Deep Neural Networks with Joint Quantization and Pruning of Features and Weights},
pdfsubject={deep learning},
pdfauthor={Xinyu Zhang},
pdfkeywords={Quantization, Neural Networks, Pruning, Feature Pruning, Software Tool, Python, Pytorch, 
Model Compression, Object Detection, Super Resolution, Classification, Image to Image
Translation, Generative Adversarial Network, CycleGAN},
}

==> include.backup1002/body.tex <==
\begin{abstract}
				
	Quantization and pruning are widely used to reduce the inference costs of
	deep neural networks, but are typically treated as independent problems. In
	this work, we empirically evaluate this independence assumption across a
	wide range of computer vision tasks and observe interdependence and
	non-commutativity when applied to both features and weights. Informed by
	these observed dependencies, we propose a novel method to jointly train deep
	neural networks using both uniform quantization and unstructured pruning on
	both the features and weights. We demonstrate that our method delivers an
	increased performance per memory footprint over existing state-of-the-art
	solutions.
				
\end{abstract}
	
	
	
\section{Introduction}
\label{sec:intro}



Convolutional neural networks (CNN) have been widely deployed in various
applications. To increase inference efficiency of CNN, quantization and sparsity
are important topics which have been studied extensively. 
Quantization \citep{n16_wu2020integer} reduces the precision required for weight
and feature, which enables us to accelerate CNN with fixed-point arithmetics and
smaller memory footprint. Quantization-aware training is an approach which
applies quantization during the training process and usually yields better
accuracy than post training quantization \citep{o_hubara2017quantized}.
Sparsity refers to a subset of model parameters have a value of exactly zero,
whose corresponding multiplication can skipped, and enables models to be stored
and transmitted using sparse matrix format. Magnitude-based weight pruning is a simple
technique that sets weights with least magnitude to zero according to some
sparsification schedule during training \citep{n35_hoefler2021sparsity}, which
is shown to deliver comparable or better results than complex techniques
\citep{n38_gale2019state}. 

% We will refer magnitude-based pruning as pruning in
% the rest of the paper.


\textbf{Non-Commutativity Hypothesis.} \textit{When quantization and pruning are
	 applied on both weights and features during training of a CNN, there exists
	an optimal temporal order between pruning and quantization, and not
	following the optimal order can lead to catastrophic performance
	degradation. Instead of having a global unique solution, this optimal order
	varies over specific tasks and neural architectures.}

Pruning and quantization are often considered to be able to solve independently
\citep{n21_liang2021pruning}. Though there have been some recent research to
study both quantization and pruning in a unified scope, they generally assume a
Prune-then-Quantize paradigm without enough investigation on other possibilities
\citep{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint}. However, we find
that the temporal order of quantization and pruning becomes a critical factor
when we apply unstructured pruning on the feature map, and we will discuss
unstructured feature sparsity in Sec.~\ref{sec:pre-feat-s}. We state
\textit{non-commutativity hypothesis} based on our results.



In the field of computer vision, existing work on quantization and pruning
mostly focus on discriminative tasks, such as image classification, object
detection instead of generative tasks like image to image translation, and
generative adversarial network (GAN). \citep{n23_wang2019qgan} proposes a weight
quantization scheme for GAN, and \citep{n34_zhou2020sparse} uses sparse
regularization to improve generative quality, while we show our method
enables to jointly quantize and prune on Pix2Pix \citep{pix2pix} and CycleGAN
\citep{o_cyclegan}.


\textbf{Contributions.}

\begin{enumerate}
	\item In Sec.~\ref{sec:non-comu}, we empirically analyze and gain many insights on
	unstructured feature pruning. Contrary to the independence assumption, we
	experimentally show non-commutativity between pruning and quantization when
	applied to both features and weights.


	\item In Sec.~\ref{sec:method}, we propose a novel method to jointly train deep neural networks using
	both uniform quantization and unstructured pruning on both the features and
	weights. We show that our method is able to deliver the best performance per memory
	footprint over existing state-of-the-art solutions.
	      	      	      
	\item In Sec.~\ref{sec:exp}, we empirically show that our method supports a wide
	      range of computer vision applications over image classification, object
	      detection, super resolution, Pix2Pix \citep{pix2pix} and CycleGAN
	      \citep{o_cyclegan}.
	      	      	      	      	      	      	      	      	      																																																																																																																																																																																																																													  
	\item We release our method as a pytorch-based python package \ourlib. In
	Appendix.~\ref{apn:software}, we demonstrate our library is compatible to
	any pytorch modules with a completely innovative design.
\end{enumerate}





% Most existing work focus on image
% classification, and some work have covered object detection
% \citep{detect_li2019fully}. However, this study has not yet but should be
% generalized to a broader range of computer vision (CV) tasks. For example,
% pruning and quantization research on generative tasks like generative
% adversarial network (GAN) is still limited to weight quantization
% \citep{n23_wang2019qgan} and sparse regularization \citep{n34_zhou2020sparse}.




\section{Preliminary}
\label{sec:pre}

Let $L \in \mathbb{N}^+$ denote the number of layers in a CNN, $f_i,
i\in\{1,...,L\}$ be the output feature map of layer $i$, $f_0$ be the CNN input, $w_i$ be the weight
of layer $i$, $T_i(f, w)$ be
the computation function of layer $i$, such as convolution,
$\sigma$ be the activation function, then a CNN can be written
as a function $Net$ in Eq.~\ref{eq:cnn}:

\vspace{-1em}


\begin{equation}
	f_L \mapsto Net(f_0) = T_L(\sigma(T_{L-1}(... \sigma(T_1(f_0, w_1)) ... )), w_L)
	\label{eq:cnn}
\end{equation}

\subsection{Uniform Quantization}
\label{sec:pre-quantize}

Suppose $x$ to be either feature or weight, uniform quantization
\citep{PEARLMAN199513} quantizes $x$ by partitioning in a equally
quantization levels as shown in Eq.~\ref{eq:uniform_q}, where $N$ be the total
number of bits, $d$ be the number of decimal bits (bits used to represent
fractions).

\vspace{-1em}


\begin{equation}
	\text{uniform\_quantize}(x, d) = \text{clip}(\floor{x * 2^{d}}, -2^N, 2^N-1) / 2^d
	\label{eq:uniform_q}
\end{equation}


To calculate gradients of uniform quantization operation, straight-through
gradient estimator (STE) \citep{o_hubara2017quantized} is usually applied for backward computation as shown in
Eq.~\ref{eq:ste}.

\vspace{-1em}


\begin{equation}
	\frac{\partial Loss}{\partial x} = \text{clip}(\frac{\partial Loss}{\partial x_q}, -2^{N-d}, 2^{N-d} - 1)
	\label{eq:ste}
\end{equation}

\subsection{Magnitude-based Weight Pruning}
\label{sec:pre-prune}

Magnitude-based weight pruning uses weight magnitude as a proxy to represent
weight importance and set least important weights to zero following a
sparsification schedule \citep{n38_gale2019state}. \citep{n45_zhu2017prune}
proposes to maintain a binary mask $m_{w_i}$ for each $w_i$ and prune $w_i$
as shown in Eq.~\ref{eq:prune}, which allows for masked weights to reactivate
during training. At inference, the mask is unnecessary and only non-zero weights
will be kept. 

\vspace{-1.5em}


\begin{equation}
	\text{prune}(w_i) = w_i m_{w_i}
	\label{eq:prune}
\end{equation}

Let $s_t(w_i)$ denote the ratio of zeros (sparsity) in $m_{w_i}$ at time $t$,
pruning starting at training step $t_0$ with pruning frequency $\Delta t$ and
$n$ pruning steps, $s_f$ be the final sparsity, \citep{n45_zhu2017prune} designs
the sparsification schedule with cubic function as shown in
Eq.~\ref{eq:to_prune}. The cubicity enables to prune rapidly in the initial
phase and slowly near the end, which empirically delivers good performance.

\vspace{-1em}

\begin{equation}
	s_{t}(w_i)=s_{f} \left(1 - \left(1-  \Bigl\lfloor\frac{t- t_0}{n \Delta t}\Bigr\rfloor\right)^{3} \right) 
	\label{eq:to_prune}
\end{equation}


Pruning is called structured if it imposes structures over the topology of the 
sparse weight (structured sparsity), which provides a trade-off
between accuracy and implementation feasibility  
because unstructured weight sparsity is difficult to efficiently implement on
contemporary GPUs \citep{n13_gray2017gpu}. \citep{wang2020structured} designs a
structured pruning method for weights and features by pruning weights in a
specific channel-wise manner. In this work, we focus on unstructured pruning
because it is most flexible and unstructured feature sparsity has the potential
to provide an inherently better trade-off than unstructured weight sparsity as
we discuss in the next section.



\subsection{Unstructured Feature Sparsity}
\label{sec:pre-feat-s}


Due to the prevalence of rectified activation functions \citep{xu2015empirical},
CNN features are inherently sparse \citep{glorot2011deep}. Except that the sparse
pattern is not pre-determined but depends on each input, thus making it
difficult to utilize during inference. In this work, we refer unstructured feature sparsity to a
subset of neurons gets removed from a neural network, whose corresponding
computations can skipped, and feature maps can be stored with fewer memory. 

\citep{hu2016network} applies post-training unstructured pruning to remove neurons by taking advantage
of existing feature sparse pattern caused by ReLU activation. Contrary to their
method, we propose to apply unstructured pruning on features during training
with an introduced sparsity instead of only leveraging existing sparse pattern,
and we study this problem in the context of quantization and weight pruning.


We argue that unstructured sparsity is more beneficial for inference on features
than weights. Taking convolution as an example, it is like having \quotes{holes}
on designated locations of a feature map whose computation can be skipped
because they will always returns zero, and skipping a single output feature
value can save an entire dot product \citep{convarith_dumoulin2016guide}. 



\section{Non-Commutativity Analysis} 
\label{sec:non-comu}

In this section, we empirically evaluate our \textit{non-commutativity
hypothesis} with image classification, object detection and super resolution
tasks with the method in Sec.~\ref{sec:method}. To fairly compare various
configurations under a unified scope, we introduce a metric called
\textit{performance density} (PD). We define the performance density of a model
as its accuracy divided by memory footprint of both parameters and feature maps in
megabits.

\textbf{Empirical Evaluation of Existing Ideas.} We start by assessing the previous Prune-then-Quantize paradigm
\citep{n8_han2015deep, n10_zhao2019focused, n17_yu2020joint} and independence
assumption \citep{n21_liang2021pruning, o_paupamah2020quantisation} between
quantization and pruning. In Table~\ref{tb:evaluate_previous}, we experiment
the settings of \quotes{joint weight pruning and weight \& feature quantization} and
explain our notation for experiment configuration. Note that
there could have many combinations over different quantization and pruning
setups, but we choose the above ones to isolate the order of these
two operations. 

We find these existing ideas hold for some cases but not all, which actually
softens their strengths. The \pq{w}{w,f} delivers the significantly better
performance than \qp{w,f}{w} for (a), which means they are not independent.
However, in (c) the order of \p{w} and \q{w,f} does not make major difference
and the difference in (b) also appears to be marginal, which indicates these two
operations are exchangeable and Prune-then-Quantize may not be strictly
required. 


\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (a) MobileNetV2}    & \textbf{Top-1 Acc} & \textbf{PD} \\ \hline
				Baseline           & 92.6    & 1          \\ \hline
				\pq{w}{w,f} & \textbf{92.23}   & 1    \\ \hline
				\qp{w,f}{w} & 85.94   & 1    \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\footnotesize
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (b) ResNet101}    & \textbf{mAP} & \textbf{PD}  \\ \hline
				Baseline              & 74.47  & 1       \\ \hline
				\pq{w}{w,f} & \textbf{74.44}  & 1 \\ \hline
				\qp{w,f}{w} & 74.13   & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (c) ESPCN}          & \textbf{PSNR} & \textbf{PD} \\ \hline
				Baseline             & 32.84   & 1      \\ \hline
				\pq{w}{w,f} & 32.51  & 1 \\ \hline
				\qp{w,f}{w} & \textbf{32.54}  & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize Comparison between the orders of \quotes{pruning and
	quantization without unstructured feature pruning} in (a) image
	classification with MobileNetV2 on CIFAR10, (b) objection detection with
	Faster RCNN and ResNet101 on Pascal VOC, and (c) super resolution with ESPCN
	\citep{espcn} on Set5 (from left to right), which empirically evaluates
	existing ideas of Prune-then-Quantize paradigm and independence assumption.
	Note that we use the notation of \pq{w}{w,f} to denote the setting that
	first prunes 50\% weight then quantizes weight and feature with 8bit, the
	same rule applies for others. }
	\label{tb:evaluate_previous}
\end{table}

\textbf{Non-Commutativity Hypothesis.} We add \quotes{unstructured feature pruning} to
the previous experiment configuration and results are shown in
Table~\ref{tb:non-comu}. We can see that feature pruning can drastically reduce
memory footprint while maintaining a similar level of accuracy, thereby has a
much higher performance density than their weight pruning counterpart. Besides,
we observe an optimal order between quantization and pruning for each setting,
and this optimal order varies among tasks. Changing the order can result in
significantly large accuracy degradation, which we conclude under our \textit{non-commutativity hypothesis}.


\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (a) MobileNetV2}    & \textbf{Top-1 Acc} & \textbf{PD} \\ \hline
				Baseline           & 92.6    & 1          \\ \hline
				\pq{w,f}{w,f} & \textbf{91.44}  & 1    \\ \hline
				\qp{w,f}{w,f} & 86.84   & 1    \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\footnotesize
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (b) ResNet101}    & \textbf{mAP} & \textbf{PD}  \\ \hline
				Baseline              & 74.47  & 1       \\ \hline
				\pq{w,f}{w,f} & \textbf{73} & 1 \\ \hline
				\qp{w,f}{w,f} & 70.13  & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (c) ESPCN}          & \textbf{PSNR} & \textbf{PD} \\ \hline
				Baseline             & 32.84   & 1      \\ \hline
				\pq{w,f}{w,f} & 31.03   & 1 \\ \hline
				\qp{w,f}{w,f} & \textbf{31.66}   & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize Comparison between the orders of \quotes{pruning and
	quantization with unstructured feature pruning}, which empirically evaluates
	the \textit{non-commutativity hypothesis}.}
	\label{tb:non-comu}
\end{table}


This observation motivates us to further investigate the properties of
unstructured feature pruning. In Table~\ref{tb:interdependence}, by comparing
\quotes{feature pruning} and \quotes{feature pruning with quantization}, we even find that
unstructured feature pruning could possibly benefit from quantization in
setting (c). Moreover, comparing \pq{w,f}{w,f} of (c) in
Table~\ref{tb:non-comu} and (c) in Table~\ref{tb:interdependence}, we find the
accuracy of \p{f} decreases at \pq{w,f}{w,f} but increases at \qp{w,f}{w,f},
which suggests the optimal order from \textit{non-commutativity hypothesis}
could even improve the accuracy of unstructured feature pruning in certain
scenarios.

Additionally, we compare the accuracy of applying \quotes{unstructured feature pruning
only} versus applying \quotes{everything else except feature pruning} in
Table~\ref{tb:degradation}. We find \p{f} has a greater negative
impact on accuracy than both \p{w} and \q{w,f} combined, but it can yields 
higher performance density in \todo{ref to certain rows after PD is computed}.


\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (a) MobileNetV2}    & \textbf{Top-1 Acc} & \textbf{PD} \\ \hline
				Baseline           & 92.6    & 1          \\ \hline
				\p{f} & \textbf{91.87}  & 1    \\ \hline
				\pq{w,f}{f} & 91.44   & 1    \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\footnotesize
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (b) ResNet101}    & \textbf{mAP} & \textbf{PD}  \\ \hline
				Baseline              & 74.47  & 1       \\ \hline
				\p{f}  & \textbf{73.04} & 1 \\ \hline
				\pq{w,f}{f} & 73  & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (c) ESPCN}          & \textbf{PSNR} & \textbf{PD} \\ \hline
				Baseline             & 32.84   & 1      \\ \hline
				\p{f} & 31.36   & 1 \\ \hline
				\qp{w,f}{f} & \textbf{32.03}    & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize Comparison between \quotes{feature pruning only} and \quotes{feature
	pruning with quantization}, the optimal order between quantization and
	pruning is used for the latter case. Task (c) shows a dependence of
	unstructured feature pruning over quantization.}
	\label{tb:interdependence}
\end{table}



\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (a) MobileNetV2}    & \textbf{Top-1 Acc} & \textbf{PD} \\ \hline
				Baseline           & 92.6    & 1          \\ \hline
				\p{f} & 91.87  & 1    \\ \hline
				\pq{w}{w,f} & \textbf{92.23}   & 1    \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\footnotesize
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (b) ResNet101}    & \textbf{mAP} & \textbf{PD}  \\ \hline
				Baseline              & 74.47  & 1       \\ \hline
				\p{f}  & 73 & 1 \\ \hline
				\pq{w}{w,f} & \textbf{74.44}  & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (c) ESPCN}          & \textbf{PSNR} & \textbf{PD} \\ \hline
				Baseline             & 32.84   & 1      \\ \hline
				\p{f} & 31.36   & 1 \\ \hline
				\qp{w,f}{w} & \textbf{32.59}    & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize 	Comparison between \quotes{feature pruning only} and \quotes{weight
	pruning and weight \& feature quantization}, which shows unstructured feature
	pruning contributes more to accuracy degradation than weight pruning and
	quantization combined, but delivers higher performance density in \todo{ref
	to certain rows when PD is computed.}}
	\label{tb:degradation}
\end{table}




\textbf{Explanation.} To understand the \textit{non-commutativity hypothesis},
we provide an explanation from the gradient perspective. In
Fig.~\ref{fig:gspike}, we find that pruning will incur spikes on gradient of
activations when operating on feature because loss will be more concentrated on
the remaining values, which could even possibly be exacerbated
through back-propagation. 


\begin{figure}[H]
	\centering
	\begin{minipage}{.33\textwidth}
		\centering
		\scalebox{0.35}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_feat.pdf}
		}
	\end{minipage}%
	\begin{minipage}{0.33\textwidth}
		\centering
		\scalebox{0.35}{
			\includegraphics{plots/pictures/grad_scale_analysis/why_prune_then_quantize/sr_grad.pdf}
		}
	\end{minipage}
	\begin{minipage}{0.33\textwidth}
		\dummyfig{gradients at a different layer}{0.1}{0.8}
	\end{minipage}
	\caption{Visualization of
	gradient spikes effect during unstructured feature pruning. More
	examples of other tasks are provided in Appendix~\ref{apn:more_exp}.}
	\label{fig:gspike}
\end{figure}



The gradient spikes could correlate with two additional dynamics: (1) the
gradient clamping behavior from straight-through gradient estimator in
Eq.~\ref{eq:ste}. (2) gradients of the origin model. For each combination of
task and neural architecture, the tension among these dynamics could behave in
completely different patterns when the order of quantization and pruning
changes, which could result in non-commutativity phenomenon.


Based on the above explanation, we suppose that the existence of
\textit{non-commutativity hypothesis} and the corresponding optimal order depend
on tasks and neural architectures. To further evaluate the validity of the
hypothesis, we apply different neural network structures for the task
configurations of Table~\ref{tb:evaluate_previous} and results are shown in
Table~\ref{tb:non-comu2}. \todo{comment on the experiment result when they are available.}

\begin{table}[]
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (a) DenseNet121}    & \textbf{Top-1 Acc} & \textbf{PD} \\ \hline
				Baseline           & 1    & 1          \\ \hline
				\pq{w,f}{w,f} & 1  & 1    \\ \hline
				\qp{w,f}{w,f} & 1   & 1    \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\resizebox{\textwidth}{!}{
			\footnotesize
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (b) VGG16}    & \textbf{mAP} & \textbf{PD}  \\ \hline
				Baseline              &  1 & 1       \\ \hline
				\pq{w,f}{w,f} & 1 & 1 \\ \hline
				\qp{w,f}{w,f} & 1  & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\begin{minipage}[t]{0.33\textwidth}
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c|c|}
				\hline
				\textbf{\small (c) SRCNN}          & \textbf{PSNR} & \textbf{PD} \\ \hline
				Baseline             & 1   & 1      \\ \hline
				\pq{w,f}{w,f} &  1  & 1 \\ \hline
				\qp{w,f}{w,f} & 1   & 1 \\ \hline
			\end{tabular}
		}
	\end{minipage}
	\caption{\footnotesize \todo{Empirical evaluation of \textit{non-commutativity hypothesis} with more neural architectures}}
	\label{tb:non-comu2}
\end{table}




\section{Joint Quantization and Pruning}
\label{sec:method}

Along with the analysis of the \textit{non-commutativity hypothesis}, we develop
a novel method that jointly quantizes and prunes both features and weights of a
CNN. Our method consists of a quantization operator and a pruning operator. The
joint pipeline is shown in Fig.~\ref{fig:pipeline}. As the uniform quantization
is symmetric around the origin, we place pruning structurally before the
quantization operator. However, contrary to previous methods which use a
determined temporal order of pruning and quantization, based on our analysis in
Sec.~\ref{sec:non-comu}, we propose to use hyper parameters to control the
temporal order of pruning and quantization.



\begin{figure}[]
	\centering
	\includegraphics[width=0.7\linewidth]{plots/conv.pdf}
	\caption{An example of applying joint pruning and quantization of both
		weight and feature on a convolution layer.}
	\label{fig:pipeline}
\end{figure}


\subsection{Quantization Operator}

\begin{figure}[]
	\begin{minipage}[t]{0.38\linewidth}
		\begin{figure}[H]
		\scalebox{0.29}{
			\includegraphics{plots/pictures/feat_histogram_analysis/together.pdf}
		}
		\caption{Feature distribution of CycleGAN and MobileNetV2 used for classification in CIFAR10.}
		\label{fig:feat_dist}
		\end{figure}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.58\linewidth}
		\begin{figure}[H]
		\scalebox{0.325}{
			\includegraphics{plots/pictures/cyclegan/saturation/3.pdf}
		}
		\caption{Generated images from CycleGAN networks, where saturated quantization is critical for generative quality.}
		\label{fig:cyclegan_demo1}
		\end{figure}
	\end{minipage} 
\end{figure}

We make two simple yet effective enhancements on top of the STE-based quantization in Sec.~\ref{sec:pre-quantize}, as
explained below. %and Alg.~\ref{alg:quantize}. 

\textbf{Delayed Quantization.} Instead of using floating point auxiliary weights
for simulated quantization \citep{n25_jacob2018quantization} or finding clever
weight initialization \citep{o_init_q}, we start by training the original float
network, then calculate the optimal decimal bits by minimizing the quantization
error after a given number of steps $t_q$. Let $x_t$ to be either feature or
weight at time $t$, our quantization operator is demonstrated in
Eq.~\ref{eq:delayed}. 

																																																																																																																																																																																																																																																	
\begin{equation}
	\small
	\text{quantize}(x_t) = \begin{cases} 
		x_t & t < t_q \\
		\text{uniform\_quantize}(x_t, d^*)  &    t \ge t_q  \text{ where $d^* = \arg \min_{d} |\text{uniform\_quantize}(x_{t_q}, d) - x_{t_q}|^2$ } \\
	 \end{cases}
	\label{eq:delayed}
\end{equation}


By thorough experiments in Sec.~\ref{sec:exp}, we show that our method achieves superior performance while
accommodating initialization and training dynamics of various tasks and network
structures.


\textbf{Saturated Quantization.} When calculating $d^*$ for feature in Eq.~\ref{eq:delayed}, we find the
quantization error minimization can be biased from outliers for tasks like
CycleGAN. In Fig.~\ref{fig:feat_dist}, we can see that the feature distribution of CycleGAN
is much more long-tailed than that of MobileNetV2 in image classification, which will result in
underestimation of $d^*$ and collapse the
generative model as shown in Fig.~\ref{fig:cyclegan_demo1}.


Therefore, instead of using the standard mean square quantization error as in Eq.~\ref{eq:delayed},
we saturate $x_{t_q}$ to protect the quantization from outliers as in
Eq.~\ref{eq:qmse}.

																																																																																																																																																																																																																																																	
\begin{equation}
\begin{split}
	d^* & = \arg \min_{d} |\text{uniform\_quantize}(\text{saturate}(x_{t_q}), d) - \text{saturate}(x_{t_q})|^2 \\
	\text{saturate}(x) & = \text{clip}(x, \text{quantile}(x, s_l), \text{quantile}(x, s_u)) \\
	\text{quantile}(x, a) & =  a\text{-th quantile of } x \\
	s_l, s_u & \in [0, 100], s_l < s_u
\end{split}
\label{eq:qmse}
\end{equation}


\subsection{Pruning Operator}

We adopt the magnitude-based weight pruning method in Sec.~\ref{sec:pre-prune}
and use it to prune features as well by maintaining a binary mask $m_{f_i}$ for
each feature map $f_i$ and prune $f_i$ as in Eq.~\ref{eq:prune}. We also make a
small enhancement by introducing a sliding window to calculate $m_{f_i}$ with
features from multiple batches. We report the impact of sliding window size on
unstructured feature pruning in Appendix~\ref{apn:more_exp}.


% We make a simple enhancement on top of the magnitude-based quantization in Sec.~\ref{sec:pre-quantize}, as
% explained below and Alg.~\ref{alg:quantize}. 
					

% for feature pruning
% The modification we make is instead of only depending on magnitude of the
% current input, during feature pruning, we maintain an input buffer so we construct the mask from the
% magnitude of a history of features. We see that the input buffer is important for
% unstructured feature pruning in Table~\ref{tb:frcnn_bf}. 





\subsection{Software Interfaces}

We release our method in a pytorch-based software package. In
Appendix~\ref{apn:software}, we demonstrate how simple and flexible it can make
pruned and quantized training to be. Unlike existing libraries
\citep{t_xilinx,QatTorch} that only provides a limited set of quantized or
pruned layers isolated from other modules, our library directly transforms the
weight attribute of the input layer into a quantized or pruned version during
runtime. This is to say, our library is layer-agnostic and can work with any
pytorch modules, as long as their parameters can be accessed from the weight
attribute. More information can be found at \ourlib.



\section{Experiments}
\label{sec:exp}

To evaluate our method, we conduct experiments on five tasks: image
classification, object detection, super resolution, image to image translation,
and generative adversarial network. We implement each task by applying minimal
code changes with our library on top of existing popular open-source
implementations. We maintain hyper-parameters identical to the original settings
except for training epochs and when to apply quantization \& pruning. More
details about experiment setups are available in
appendix~\ref{apn:detailed_exp}. We release all experiment source code as
examples for our library.

\textbf{Image Classification.} We conduct our image classification task on
CIFAR10 \citep{o_cifar10} with MobileNetV2 \citep{mobilenetv2} and DenseNet121
\citep{huang2017densely}. We compare with previous methods in
Table~\ref{tb:cifar10_comp}.



					

\begin{table}[]
	\centering
	\vspace{-1em}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccccccccc}
			\toprule
			Method
			& Network                                           & W Bits
			& F Bits                   & W Sparsity                  & F
			Sparsity                & Ref Acc                               &
			\multicolumn{1}{c}{Accuracy}  & \multicolumn{1}{c}{\scriptsize \begin{tabular}[c]{c}Mem (Mb) \end{tabular}} &
			\multicolumn{1}{c}{\scriptsize \begin{tabular}[c]{c}PD (Acc/Mb)
			\end{tabular}}   \\
			\midrule
			\multicolumn{1}{c|}{\script{\citep{n40_choi2016towards}}}
			& \multicolumn{1}{c|}{ResNet-32}                    &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{77.8\%} & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.58}                 & 92.64 (+0.06)    &
			168.87 & 0.55			\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n44_achterhold2018variational}}}
			& \multicolumn{1}{c|}{DenseNet-76}                  &
			\multicolumn{1}{c|}{2}    & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.19}                 & 91.17 (-1.02)  &
			283.21 & 0.32                 \\ \midrule
			
			\multicolumn{1}{c|}{\multirow{3}{*}{\script{\citep{n29_liu2018rethinking}}}}
			& \multicolumn{1}{c|}{VGG-19}                       &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{80\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.5}                  & 93.52 (+0.02)       &
			167.06 & 0.56          \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{PreResNet-110}                &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.04}                 & 95.06 (+0.02) &
			1571.74 & 0.06             \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{DenseNet-100}                 &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{30\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.24}                 & 95.21 (-0.03)  &
			453.84 & 0.21                \\ \midrule
			
			\multicolumn{1}{c|}{\script{\citep{n43_zhao2019variational}}} & \multicolumn{1}{c|}{DenseNet-40} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{59.67\%} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{94.11} 
			& 93.16 (-0.95)    & 118.10 & 0.79               \\ \midrule

			
			\multicolumn{1}{c|}{\script{\citep{n3_xiao2019autoprune}}}
			& \multicolumn{1}{c|}{VGG-16}                       &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{79\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.4}                  & 91.5 (-1.9)        &
			134.36 & 0.68		\\ \midrule

			\multicolumn{1}{c|}{\multirow{2}{*}{\script{\citep{n33_dettmers2019sparse}}}}
			& \multicolumn{1}{c|}{VGG16-C}                      &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.51}                 & 93 (-0.51)   &  58.96 & 1.58                  \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{WRN-22-8}                     &
			\multicolumn{1}{c|}{--}   & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{95\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{95.74}                 & 95.07 (-0.67)     &
			258.15 & 0.37		\\ \midrule
		

			\multicolumn{1}{c|}{\script{\citep{n2_yang2020automatic}}}
			& \multicolumn{1}{c|}{ResNet-20}                    &
			\multicolumn{1}{c|}{1.9}  & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{54\%}   & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{91.29}                 & 91.15 (-0.14)  & 88.41
			& 1.03  \\ \midrule

			\multicolumn{1}{c|}{\script{\citep{n4_van2020bayesian}} }
			& \multicolumn{1}{c|}{VGG-7}                        &
			\multicolumn{1}{c|}{4.75} & \multicolumn{1}{c|}{5.4} &
			\multicolumn{1}{c|}{--}    & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{93.05}                 & 93.23 (+0.18)
			&  47.12 & 1.98		\\ \midrule
			\multicolumn{1}{c|}{\script{\citep{n24_paupamah2020quantisation}}}
			& \multicolumn{1}{c|}{MobileNet}                    &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{91.31}                 & 90.59 (-0.72)        &
			38.91 & 2.33		\\ \midrule
			
			
			\multicolumn{1}{c|}{\script{\citep{n41_choi2020universal}}}
			& \multicolumn{1}{c|}{ResNet-32}                    &
			\multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{--}  &
			\multicolumn{1}{c|}{87.5\%}  & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{92.58}                 & 92.57 (-0.01)    &
			152.35 & 0.61			\\ \midrule
			
			\multicolumn{1}{c|}{\multirow{4}{*}{Ours}}
			& \multicolumn{1}{c|}{\multirow{2}{*}{MobileNetV2}} &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{\multirow{2}{*}{92.6}} &
			\multicolumn{1}{c}{92.23 (-0.37)} & 64.39 & 1.43 \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{}                             &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{50\%} &
			\multicolumn{1}{c|}{}                      &
			\multicolumn{1}{c}{91.44 (-1.16)} &  \textbf{36.79} & \textbf{2.49}
			\\
			
			\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\multirow{2}{*}{DenseNet121}} &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{--}   &
			\multicolumn{1}{c|}{\multirow{2}{*}{1}} &
			\multicolumn{1}{c}{1} & 1 & 1 \\
			\multicolumn{1}{c|}{}
			& \multicolumn{1}{c|}{}                             &
			\multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{8}   &
			\multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{50\%} &
			\multicolumn{1}{c|}{}                      &
			\multicolumn{1}{c}{1} &  1 & 1 \\ \bottomrule
		\end{tabular}
	} 
					
	\caption{Comparisons with previous pruning or quantization methods on
	CIFAR10. Our method is able to deliver the smallest memory footprint and best
	performance density and is far more versatile.}
	\label{tb:cifar10_comp}
\end{table}




\textbf{Object Detection.} 
We conduct our objection detection experiment on Pascal VOC \citep{o_pascalvoc}
using Faster RCNN \citep{o_fasterrcnn} with a ImageNet \citep{o_imagenet}
pre-trained ResNet101 and VGG16 backbone. Results can be found in
Table~\ref{tb:non-comu} and \ref{tb:non-comu2}.
Since the original Faster RCNN trains on images of different shapes each batch,
it is impossible to obtain a fixed binary mask for convolution output. Thus, we apply channel-wise
pruning on convolution feature. Note that we do not prune or quantize for the
first 5 residual blocks because they are frozen originally and unfreezing will
collapse the training even for float dense network. However, this limitation can
be easily overcome with group normalization or synchronized batch normalization
according to \citep{he2019rethinking}. Thus, we do not regard this as our
limitation. Contrary to existing methods like \citep{detect_li2019fully}, which
introduces major overhauls over the object detection network training
procedures, our method is less intrusive and works without much modifications.
Aligning with the original setting, we train with batch size equal to 1 and fix
all pre-trained batch normalization layers.

\textbf{Super Resolution.} 
We conduct our super resolution task on 91-image \citep{o_91image} (training
set) and Set5 \citep{o_set5} (validation set) with efficient sub-pixel
convolution network (ESPCN) \citep{espcn} and SRCNN \citep{dong2015image}, both
are 3-layer convolution networks without normalization layer. Results can be
found in Table~\ref{tb:non-comu} and \ref{tb:non-comu2}. Though every
configuration suffers a performance drop, the result of \pq{w,f}{w} almost has
the identical PSNR with the original result reported in \citep{espcn}.
\citep{ayazoglu2021extremely} also quantizes and evaluates ESPCN against Set5,
but it uses pre-trained weights from ImageNet while we train from scratch, so we
do not regard them as our comparison.

\begin{figure}[]
	\begin{minipage}[t]{0.48\linewidth}
		\scalebox{0.265}{
			\includegraphics{plots/pictures/pix2pix/both/24.pdf}
		}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.48\linewidth}
		\vspace{-4.25em}
		\scalebox{0.265}{
			\includegraphics{plots/pictures/cyclegan/both/3.pdf}
		}
	\end{minipage} 
	\caption{Examples of generated images from Pix2Pix (left) and CycleGAN
	(right) networks.}
	\label{fig:pix2pix_cyclegan}
\end{figure}



\begin{table}[]
	\centering
	\begin{minipage}[t]{0.4\linewidth}
		% \flushright
		% \resizebox{\textwidth}{!}{
			\begin{table}[H]
				\begin{tabular}{|l|l|l|}
				\hline
				\textbf{Pix2Pix} & \textbf{IS} & \textbf{PD}  \\ \hline
				Baseline         & 1     & 1         \\ \hline
				\pq{w}{w,f}      & 1     & 1         \\ \hline
				\pq{w,f}{w,f}    & 1      & 1        \\ \hline
				\end{tabular}
			\end{table}
		% }
	\end{minipage}%
	% \hfill%
	\begin{minipage}[t]{0.4\linewidth}
		% \resizebox{\textwidth}{!}{
			\begin{table}[H]
				\begin{tabular}{|l|l|l|}
				\hline
				\textbf{CycleGAN} & \textbf{IS} & \textbf{PD} \\ \hline
				Baseline         & 1          & 1    \\ \hline
				$P_{0.5}(w)\rightarrow Q_{12}(w,f)$      & 1   & 1        \\ \hline
				$P_{0.5}(w,f)\rightarrow Q_{12}(w,f)$    & 1   & 1        \\ \hline
				\end{tabular}
			\end{table}
		% }
	\end{minipage} 
	\caption{\todo{Inception Scores (IS) of Pix2Pix and CycleGAN with different training configurations.}}
	\label{tb:is}
\end{table}

\textbf{Pix2Pix and CycleGAN.} We conduct our image to image translation task on
facades dataset with Pix2Pix network \citep{pix2pix}, and our GAN task on
horse2zebra dataset with CycleGAN \citep{o_cyclegan}. Both of them applies an
encoder-decoder structured network, while the Pix2Pix uses UNet \citep{unet} and
CycleGAN uses a variant of ResNet with deconvolution layers. Some generated
samples are demonstrated in Fig.~\ref{fig:pix2pix_cyclegan} and inception scores
\citep{borji2019pros} are shown in Table~\ref{tb:is}. We provide more samples in
appendix~\ref{apn:more_demos}. For Pix2Pix, it is hard to distinguish the
quality difference between samples of baseline and \pq{w}{w,f}. If we add
feature pruning, though the overall structure remains, the color becomes
unnatural and some major distortions could be spotted. For CycleGAN, we find the
feature map needs more than 8bit (we use 12bit) to deliver decent generative
results. 


\section{Limitations and Future Work}

\todo{add later}
% the finding is limited to our method
% smaller datasets due to resource constraint
% TODO

\section{Related Work}

\todo{add later}

==> include.backup1002/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[strings]{underscore}
% \usepackage{url}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{bbold}
\usepackage{graphicx}

\usepackage{fancybox}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage[noend,algoruled,linesnumbered, rightnl]{algorithm2e}
\usepackage{seqsplit}
\usepackage{multirow}
\usepackage{float}
\usepackage{doi}
\usepackage{pgfplots}
\usepackage{pgf}
\usepackage{calc}  
\usepackage{array}
\usepackage{enumitem}  
\usepackage{geometry}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{multicol}
\usepackage{caption}
\usepackage{minted}
\usepackage{subcaption}
\usepackage{accents}
% \usepackage{algcompatible}
% \algnewcommand{\lst}{\texttt{lst}}
% \algnewcommand{\slst}{\texttt{slst}}
% \algnewcommand{\SEND}{\textbf{send}}

% \newsavebox{\algleft}
% \newsavebox{\algright}

\newtheorem{theorem}{Theorem}

\renewcommand{\url}[1]{\texttt{\seqsplit{#1}}}

\usepackage{tikz}
\usepackage{adjustbox}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rflo, rightnl}
\newcommand\tocite[1]{\textcolor{blue}{[#1]}}
\newcommand{\comment}[1]{}
\long\def\/*#1*/{}

\newenvironment{fminipage}%
{\begin{Sbox}\begin{minipage}}%
{\end{minipage}\end{Sbox}\fbox{\TheSbox}}


\newcommand{\python}[1]{
\inputminted[
frame=single,framesep=10pt,
bgcolor=lightergray,
fontsize=\footnotesize,
]{python}{#1}
}
\newcommand{\dummyfig}[3]{
  \centering
  \fbox{
    \begin{minipage}[c][#2\textheight][c]{#3\textwidth}
      \centering{#1}
    \end{minipage}
  }
}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\SetKwInput{KwInput}{Input} % just a guess
\SetKwInput{KwOutput}{Output} % just a guess
\definecolor{lightergray}{RGB}{242, 242, 242}

\newcommand{\bsquare}{{\scriptsize $\blacksquare$}}
\newcommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\let\includegraphicsWithoutPath\includegraphics
\renewcommand{\includegraphics}[2][]{\includegraphicsWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}

\newcommand{\quotes}[1]{``#1''}

\newcommand{\ourlib}{\href{https://github.com/anonymous368/qsparse}{https://github.com/anonymous368/qsparse}}

\newcommand{\ourexamples}{\href{https://github.com/anonymous368/qsparse/tree/main/examples}{https://github.com/anonymous368/qsparse-examples}}

\newcolumntype{T}{>{\tiny}c}
\newcolumntype{S}{>{\scriptsize}c}

\newcommand{\script}[1]{{\scriptsize #1}}

\newcommand{\pq}[2]{{\small $P_{0.5}(#1)\rightarrow Q_8(#2)$}}

\newcommand{\qp}[2]{{\small $Q_8(#1)\rightarrow P_{0.5}(#2)$}}

\newcommand{\p}[1]{{\small $P_{0.5}(#1)$}}

\newcommand{\q}[1]{{\small $Q_8(#1)$}}

\newcommand{\todo}[1]{\textcolor{red}{#1}}
